ODIN: A Single Model for 2D and 3D Segmentation

State-of-the-art models on contemporary 3D segmentation benchmarks like ScanNet consume and label dataset-provided 3D point clouds, obtained through post processing of sensed multiview RGB-D images. They are typically trained in-domain, forego large-scale 2D pre-training and outperform alternatives that featurize the posed RGB-D multiview images instead. The gap in performance between methods that consume posed images versus post-processed 3D point clouds has fueled the belief that 2D and 3D perception require distinct model architectures. In this paper, we challenge this view and propose ODIN (Omni-Dimensional INstance segmentation), a model that can segment and label both 2D RGB images and 3D point clouds, using a transformer architecture that alternates between 2D within-view and 3D cross-view information fusion. Our model differentiates 2D and 3D feature operations through the positional encodings of the tokens involved, which capture pixel coordinates for 2D patch tokens and 3D coordinates for 3D feature tokens. ODIN achieves state-of-the-art performance on ScanNet200, Matterport3D and AI2THOR 3D instance segmentation benchmarks, and competitive performance on ScanNet, S3DIS and COCO. It outperforms all previous works by a wide margin when the sensed 3D point cloud is used in place of the point cloud sampled from 3D mesh. When used as the 3D perception engine in an instructable embodied agent architecture, it sets a new state-of-the-art on the TEACh action-from-dialogue benchmark. Our code and checkpoints can be found at the project website (https://odin-seg.github.io).

==> 4_exp_Ayush.tex <==
\section{Experiments}

\subsection{Evaluation on  3D benchmarks}
% \todo{Add open vocabulary works}
\input{tables/real_in_domain_3d}

First, we benchmark our model against state-of-the-art 3D models on  ScanNet~\cite{scannet} and Scannet200~\cite{scannet200}, both for instance and semantic segmentation. The objective in these benchmarks is to label the point cloud sampled from the mesh of a scene reconstructed from raw sensor data. ScanNet200 extends ScanNet by benchmarking on 200 classes with a long-tail distribution instead of the 20 common classes used in ScanNet. Most SOTA methods directly feed the mesh-sampled point cloud to their model. However, many applications require direct processing of the raw data without going through an expensive mesh creation process. Moreover, as motivated before, utilizing RGB-D input can enable us to more closely unify 2D and 3D perception and benefit from pre-trained features and abundant 2D data. Motivated by this, we benchmark state-of-the-art 3D models in the setup where the input to their model is a point cloud obtained by directly unprojecting the raw sensor data. We also compare all models in the original setup where mesh point clouds are available. 

\paragraph{Evaluation metrics:} We follow the standard evaluation metrics, namely mean Average Precision (mAP) for instance segmentation and mean Intersection over Union (mIoU) for semantic segmentation.






%We first compare our model with state-of-the-art 3D models in popular established benchmarks of ScanNet~\cite{scannet} and Scannet200~\cite{scannet200} for instance and semantic segmentation tasks in Tables-\ref{tab:established_3d}. In these benchmarks, the task is to label the pointcloud sampled from the mesh of a scene reconstructed from the raw sensor data. 
% The results are presented in Tables-\ref{tab:established_3d}. 
% We draw the following conclusions: 

% \begin{itemize}

\textbf{Performance drops with sensor point cloud as input} (Table~\ref{tab:scannet_ins}): SOTA Mask3D's performance drops from 55.2\% mAP with mesh point cloud input to 43.9\% mAP with sensor point cloud input. This is consistent with prior works~\cite{virtualview,deepview} in 3D semantic segmentation on ScanNet, which attributes the drop to misalignments caused by noise in camera poses, depth variations and post-processing steps.

\textbf{\model{} outperforms SOTA 3D methods with sensor point cloud input} (Table~\ref{tab:scannet_ins}): Our model with Swin-Base (Swin-B) backbone significantly outperforms SOTA Mask3D model with sensor point cloud input by 4.1\%, 9.2\% and 13.6\% in mAP, mAP50 and mAP25 respectively. Our model achieves comparable performance to methods using mesh-sampled point cloud input, particularly on the mAP25 metric.
    
\textbf{\model{} sets a new SOTA in semantic segmentation on ScanNet} (Table~\ref{tab:scannet_sem}): our model outperforms all methods operating over sensor RGB point cloud including the recent Deep View Aggregation~\cite{deepview}. Additionally, our model closely matches the performance of the Virtual Multiview Fusion method~\cite{virtualview}, which generates RGB-D images from the provided mesh, incorporates design heuristics for camera view sampling to avoid occlusions, ensures balanced scene coverage, and employs higher field-of-views.$^\dagger$ \let\thefootnote\relax\footnotetext{$^{\dagger}$their code/data is not publicly available} Notably, our model also closely matches SOTA methods utilizing mesh-sampled point cloud. \nikos{why do we need this?} We also compare with OpenScene~\cite{openscene}, a state-of-the-art zero-shot 3D semantic segmentation model that uses 2D features from LSeg~\cite{lseg} and OpenSeg~\cite{openseg}. This is a zero-shot method in contrast to fully-supervised approach to ours, thus making the comparison unfair, but we include it for completeness.
    
\textbf{\model{} sets a new instance segmentation SOTA on the long-tailed ScanNet200 dataset} (Table~\ref{tab:scannet200_ins}): our model outperforms SOTA Mask3D with sensor point cloud input by 14.5\% mAP. It also outperforms SOTA mesh-point-cloud-based methods including very recent works of QueryFormer~\cite{queryformer} and MAFT~\cite{maft} by 0.8\% mAP, 4.8\% mAP50 and 7.6\% mAP25 establishing a new SOTA on this benchmark while exclusively utilizing sensor RGB-D data. This highlights the contribution of 2D features, particularly in detecting a long tail of class distribution where limited 3D data is available. We show more detailed results with performance on the head, common and tail classes in supplementary. \nikos{why do we need this?} We also compare with OpenMask3D~\cite{openmask3d}, a state-of-the-art zero-shot 3D instance segmentation model using CLIP~\cite{clip} 2D features. Note that our approach is fully supervised, making the comparison unfair, but we include it for completeness.

\textbf{\model{} sets a new semantic segmentation SOTA on ScanNet200} (Table~\ref{tab:scannet200_sem}), outperforming SOTA semantic segmentation models that use mesh point clouds by 5.6\%.
    
    \todo{We should indeed check if the major gains are in the long tail classes}
    
    %We observe that our model outperforms SOTA Mask3D in the sensor pointcloud setup by X\% and even outperforms the models trained on mesh pointcloud by Y\%, thus setting a new state-of-the-art in this benchmark. This indicates that 2D features can significantly help when tasked with detecting a long-tail of class distribution where we do not possess a lot of 3D data.
% \end{itemize}

% \todo{CAUTION: GARBAGE Ahead!}
\input{tables/ai2thor}

\subsection{Evaluation on multiview RGB-D in simulation}
As highlighted earlier, misalignments between sensor RGB-D and mesh-sampled pointclouds can significantly impact performance. Conventional 3D datasets, such as ScanNet~\cite{scannet, scannet200}, annotate the 3D mesh directly and project annotations onto sensor RGB-D images. However, these RGB-D labels inherit misalignment issues and noise due to the sparser mesh compared to RGB-D images, thus making them unsuitable for training and evaluation. To overcome this, we collect RGB-D data in the popular Ai2Thor~\cite{ai2thor} embodied simulation environment using procedural homes generated by ProcThor~\cite{procthor}. Our dataset comprises 1500 scenes, divided into 1200 training and 300 test scenes to maintain a dataset size comparable to ScanNet~\cite{scannet}. By randomly placing a robot agent at navigable locations from the simulator, we record RGB-D and camera information, facilitating the study of perception in RGB-D setups without misalignment issues.

We train and evaluate our model and SOTA Mask3D~\cite{mask3d} on the unprojected RGB-D images. As shown in Table-\ref{tab:sim}, our model outperforms Mask3D by 7\% mAP, showing strong performance in a directly comparable RGB-D setup. Despite the 2D features being pre-trained on real-world data, traditionally considered less beneficial in simulated environments, our architecture leverages pre-trained features effectively. This improvement underscores the potential of unified 2D-3D architectures in enhancing 3D perception. It suggests that current real-world benchmarks may restrain these models due to misalignments. We hope this encourages the community to also focus on directly collecting, labeling, and benchmarking RGB-D sensor data. %In supplementary, we show that we improve performance on categories common with ScanNet dataset as well

%As highlighted in the previous section, the misalignments between the sensor RGB-D and mesh sampled pointcloud can result in a sharp decrease in performance. Most popular real-world 3D datasets annotate the 3D mesh directly and project these annotations to the sensor RGB-D images. However, these RGB-D labels inherit the misalignment issues and additionally have noises due to the mesh being much sparser than the RGB-D images making them unsuitable for training and benchmarking on their RGB-D data. Thus, to study perception in RGB-D setup directly independent of the misalignment issues, we generate a scannet scale data of 1300 train scenes and 300 validation scenes from ProcThor~\cite{procthor} which is based on Ai2Thor~\cite{ai2thor} a popular simulation environment in embodied AI community. We spawn a robot agent randomly at the simulator provided navigable locations and record the RGB-D information and camera information.

%We train and evaluate our model and SOTA Mask3D on the unprojected RGB-D images. We observe that our model outperforms Mask3D by 7\% mAP showing strong performance in a comparable RGB-D setup. 

\subsection{3D perception for embodied agents in simulation}
\input{tables/teach}
% \todo{NEEDS REFINEMENT} \\
\input{tables/joint_2d_3d}
\input{tables/ablations_alt}

% \todo{also explain, seen and unsene splits of these datasets, and motivate that mesh reconstruction is not really possible or practical}
We apply our model in embodied setups (TEACh~\cite{teach} and Alfred~\cite{alfred}) in a setup where agents have depth and camera poses. In TEACh's Trajectory from Dialogue (TfD) setup, agents follow dialogues to perform tasks, while in Alfred they execute high/low-level instructions. A critical component for successful execution is object detection. Prior SOTA embodied methods~\cite{helper,film} use single-view object detectors and heuristic-based object trackers to link 2D instances into a 3D semantic map. We replace these with \model{} trained for instance segmentation on the training set of TEACh~\cite{teach}, processing the last 10  egocentric views of the agent trajectory and adding the predicted instances to the 3D semantic map of HELPER~\cite{helper}. We use Task Success Rate (SR) to assess if the agent completes the entire task and Goal Conditioned Success Rate (GC) to evaluate the proportion of goal conditions satisfied across all episodes following standard evaluation protocols~\cite{alfred, teach}. Evaluation is performed on both "valid-seen" (similar to the training set) and "valid-unseen" (different houses) splits. In Table-\ref{tab:embodied}, we observe that using \model{} significantly boosts SOTA success rate of HELPER by 2.8\% in the unseen validation split TEACh and by 10.3\% in Alfred's unseen validation split. 

%processing multiple views directly for 3D instance segmentation. We utilize \model{} on the last 10 egocentric views of the agent trajectory to obtain object instances. 


%We study an application of our perception model in the embodied setup of TEACh~\cite{teach} and Alfred~\cite{alfred} in the setup where agents have access to depth and camera poses from the simulator. We evaluate on the Trajectory From Dialogue (TfD) setup of TEACh, where the agent follows a dialogue between two human annotators to complete a given task in an embodied environment like ``Make a sandwich". The Alfred benchmark similarly evaluates the agent's ability to carry out high-level (“Rinse off a mug and place it in the coffee maker”) and low-level (“Walk to the coffee maker on the right”) instructions provided by a user. A critical component for successful execution is object detection. Prior SOTA methods on TEACh like HELPER~\cite{helper} use single-view object detectors to detect objects and a heuristic-based object tracker to link instances of a particular object to build a 3D semantic map of the scene. Since, the agent is inherently embodied and naturally has access to multiple views, we replace the single-view object detector and tracker from HELPER with \model{}, which can process multiple views and directly produce instance segmentations in 3D.
%Specifically, we run \model{} on the last 10 egocentric views of the agent trajectory to obtain a set of object instances based on multiple viewpoints. These instances are added to the 3D semantic map of the scene to be used for object navigation and interaction necessary to carry out the instruction following Helper~\cite{helper}. 
%\textbf{Evaluation Metrics} Following standard evaluation protocols~\cite{alfred, teach}, we employ the following metrics a) \textit{Task success rate (SR)} which evaluates if the agent successfully completed the entire task. b) \textit{Goal Conditioned Success Rate (GC)} which evaluates the proportion of goal conditioned achieved across all episodes. We evaluate all models on ``valid-seen" and ``valid-unseen" splits, where valid-seen comprises houses similar in distribution to train set, while ``valid-unseen" have different houses. 
%In Table-\ref{tab:embodied}, we compare Helper~\cite{helper} with \model{} as its perception system as a replacement to its single-view object detector and heuristic-based tracker. Using \model{} significantly boosts SOTA success rate of Helper by 2.8\% in the unseen validation split TEACh and by 10.3\% in Alfred's unseen validation split. 

% \todo{gabe; what do we do specifically? how many images do we process? how do we handle dynamic objects? any other useful detail?}

%\textbf{Evaluation Metrics} Following standard evaluation protocols~\cite{alfred, teach}, we employ the following metrics a) \textit{Task success rate (SR)} which evaluates if the agent successfully completed the entire task. b) \textit{Goal Conditioned Success Rate (GC)} which evaluates the proportion of goal conditioned achieved across all episodes. %Additionally, we provide path-length-weighted variants, where the weights are determined by the ratio of the expert trajectory's path length to the agent's taken path length.






\subsection{Joint 2D-3D Training}

% \todo{needs refinement}
\model{} is designed to generate segmentation masks for both single 2D RGB images and multiview RGB-D image sequences, while sharing the majority of parameters. Table~\ref{tab:joint} shows results when jointly training with 3D data from ScanNet~\cite{scannet} and 2D data from COCO~\cite{coco}. %We interleave 2D and 3D batches during training. 
We compare our model to a variant trained independently on 2D or 3D data. We find that joint training yields a 2.6\% improvement in 3D, accompanied by a slight drop in 2D. While training the model we observe that the performance on COCO continues to improve, whereas on ScanNet it starts to decline much earlier. This highlights the need to explore smarter strategies for balancing 2D and 3D data during training to prevent overfitting to one domain over the other.







%We notice that \model{} on COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other.

%Note that the 3D \model{} trained on Scannet only (in row 3) starts from pre-trained weights from Mask2Former~\cite{m2f} trained on COCO. The additional boost with joint-training suggests that it can improve performance in 3D by helping the model not to overfit on the 3D RGB-D images. We notice that COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other. Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.


%Given the higher resolution of COCO images (1024 X 1024) compared to Scannet images (256 X 256), we randomly downsample COCO images to 256 X 256 for data augmentation, aligning the 2D and 3D image resolutions. 
%We compare our model to our model's variant trained independently on 2D and 3D data. We find that joint training yields a 1.4\% improvement in 3D performance, accompanied by a slight drop in 2D performance. Note that the 3D \model{} trained on Scannet only (in row 3) starts from pre-trained weights from Mask2Former~\cite{m2f} trained on COCO. The additional boost with joint-training suggests that it can improve performance in 3D by helping the model not to overfit on the 3D RGB-D images. We notice that COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other. Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time. %We show Odin's performance when we take the best checkpoint in individual domain. 

%Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.

%This suggests that joint training 3D models with 2D data can improve performance even . Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.


%We design our architecture to handle both 2D and 3D data while sharing majority of the parameters. In this section, we train our model jointly on 3D data from scannet and 2D dataset from COCO. During training, we interleave sampling batches from 2D and 3D data. Since the images in COCO are at higher resolution of 1024 X 1024, while the scannet images are at 256 X 256 resolution, we randomly downsample COCO images to 256 X 256 as a data augmentation to match the 2D and 3D image resolutions. We compare our model against a variant of our model trained independently on 2D and the 3D data. We find that joint training helps 3D performance by 1.4\% while incurring slight performance drop in 2D. This indicates that jointly training 3D models with 2D data can help fight overfitting and improve validation performance. More importantly, we have a single unified model that, at test time, can produce segmentation masks over either single 2D RGB image or multiview RGB-D images. 
% Analysis:
% 1) sim versus real-> inaccuracy of poses
% 2) sensed mesh versus given mesh:huge difference in the numbers
% 3) long tail discussion!
% 4) virtual views: 


\subsection{Ablations}


\textbf{Cross-View fusion is crucial for instance segmentation but not for semantic segmentation} (Table~\ref{tab:cross_view}): removing cross-view contextualization layers results in a 6.9\% mAP drop for instance segmentation, while only causing a 1.3\% mIoU drop in semantic segmentation. Recent 3D open-vocabulary works~\cite{conceptfusion,openscene} without strong cross-view fusion only focus on semantic segmentation and thus could not uncover this issue. Row-3 shows a 5.7\% mAP drop when cross-view fusion happens after all within-view 2D layers instead of interleaving the within-view and cross-view fusion. This aligns with the observation from Deep View Aggregation~\cite{deepview} that early fusion is beneficial.

%\textbf{Interleaving within- and cross-view fusion is important} (Table~\ref{tab:where_cross}): row-2 shows a 5.7\% mAP drop when cross-view fusion happens after the image is processed using the full backbone instead of interleaving the within-view and cross-view fusion. This aligns with the observation from Deep View Aggregation~\cite{deepview} that early fusion is beneficial. Moreover, performing fusion only in the backbone, excluding upsampling layers, results in a 2\% performance drop (row-3), highlighting the importance of additional fusion layers to maintain feature consistency across views after 2D operations.

\textbf{Starting from pre-trained weights boosts performance} (Table~\ref{tab:pretrain}): initializing only the image backbone with pre-trained weights, instead of using all shared layers, results in a 4.7\% mAP drop (row-2). Starting the entire model from scratch leads to a larger drop of 9.1\% mAP (row-3). This underscores the importance of sharing as many parameters as possible with the 2D models to leverage their pre-trained weights effectively.

\textbf{Fine-tuning with stronger 2D backbones increases performance} (Table~\ref{tab:backbone_frozen}): using Swin-B over ResNet-50 leads to performance gains, suggesting that \model{} can directly benefit from advancements in 2D computer vision. However, this gain is not obvious when the backbone is frozen. Specifically, freezing the ResNet-50 backbone shows similar mAP performance with a 0.6\% mIoU drop, while for Swin, freezing results in a 2.4\% mAP drop and 1.3\% mIoU drop. Intuitively, unfreezing the backbone allows 2D layers to adapt to cross-view fused features better and Swin-B benefits more from this adaptation. Therefore, we keep our backbone unfrozen in all experiments.

\textbf{Supplying 2D features directly to 3D models provides no benefit:} Incorporating 2D features alongside XYZ+RGB in Mask3D yields 53.8 mAP performance comparable to 53.3\%\let\thefootnote\relax\footnotetext{$^{\dagger}$We do not use DB-SCAN post-processing of Mask3D, and hence baseline Mask3D gets 53.3 instead of 55.2 as reported by their paper} of the baseline model lacking access to 2D features.

%We unproject 2D features from Resnet-50 and supply it as an additional input to Mask3D. We find that it results in a marginal increase in task performance. Thus, while always using 2D features might be a good idea, directly supplying these features to a 3D backbone might not be an optimal design as also shown by our 2nd ablation bullet. 

% \todo{Mention DBSCAN}

% \todo{1. no alternating. sharing weights and alternating 2d 3d, do we have this number?}
% \todo{2. no cross view fusion}
% \todo{joint 2d 3d}
% \todo{many 3d}
% \todo{2d backbone variation}
% \todo{no 2d pretraining}
% \todo{straightforward addition of 2d feats to mask3d}

% \subsection{zero shot??}





% \todo{make sure we bold numbers on tables}
% \begin{table}
% \caption{\textbf{Comparison on Scannet for Instance Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llccccc}

% Input & Model & mAP &  mAP50 & mAP25 \\ \hline
% \multirow{4}{*}{Sensor RGBD PointCloud} & Mask3D $^{\dagger}$ & 43.9 & 60.0 & 69.9  \\
%  & Ours-Resnet50 & 45.7 & 66.3  & 81.8  \\
%  % & Ours-Swin-T &  &  &   \\
%  & Ours-Swin-L & 48.0 & 69.2 & 83.5  \\ \hline
% \multirow{2}{*}{Mesh Sampled Pointcloud} & SoftGroup & 46.0 & 67.6 & 78.9 \\
% & Mask3D & 55.2 & 73.7 & 83.5 \\
%  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table}
% \caption{\textbf{Comparison on Scannet for Semantic Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llc} 
% Input & Model & mIoU \\ \hline
% \multirow{8}{*}{Sensor RGBD PointCloud} 
% & MVPNet & 68.3\\
% & BPNet & 69.7 \\
% & DeepViewAgg & 71.0 \\
%  & Ours-Resnet50 & 73.2  \\
%  % & Ours-Swin-T &    \\
%  & Ours-Swin-L & 76.0 \\ \hline
% \multirow{2}{*}{Rendered RGBD PointCloud} & VMVF & 76.4 \\
% & Ours & \\ \hline
% \multirow{2}{*}{Mesh Sampled Pointcloud} & Point Transformer v2 & 75.4 \\
% & Swin3D-L & 76.7  \\
%  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table*}
% \caption{\textbf{Comparison on Scannet200 for Instance Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{llcccccccccccc}

% Input & Model & \multicolumn{3}{c}{All} &  \multicolumn{3}{c}{Head} & \multicolumn{3}{c}{Common} & \multicolumn{3}{c}{Tail} \\
%  \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}  
% & & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25\\ \midrule
% \multirow{3}{*}{Sensor RGBD PointCloud} & Mask3D $^{\dagger}$ & 15.5 & 21.4 & 24.3 & 21.9 & 31.4 &  37.1 & 13.0 & 17.2 & 18.9 & 7.9 & 10.3 & 11.5 \\
%  & Ours-Resnet50 & 26.0 & 37.6 & 43.8 &  &  &  &  &  &  &  &  &  \\
%  % & Ours-Swin-T &  &  &   \\
%  & Ours-Swin-L (in progress) &     &         &   &  & & &   \\ \midrule
% \multirow{1}{*}{Mesh Sampled Pointcloud} & Mask3D & 27.4 & 37.0  & 42.3 \\
%  \midrule
% \end{tabular}
% }
% \end{table*}


% \begin{table}
% \caption{\textbf{Comparison on Scannet200 for Instance Segmentation Task}}

% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llccc}

% Input & Model  & mAP &  mAP50 & mAP25 \\ \midrule
% \multirow{3}{*}{Sensor RGBD PointCloud} & Mask3D $^{\dagger}$ & 15.5 & 21.4 & 24.3  \\
%  & Ours-Resnet50 & 26.0 & 37.6 & 43.8  \\
%  & Ours-Swin-L &  30.0        &  43.0         &  51.0   \\ \midrule
% \multirow{1}{*}{Mesh Sampled Pointcloud} & Mask3D & 27.4 & 37.0  & 42.3 \\
%  \midrule
% \end{tabular}
% }
% \end{table}





% \todo{Maybe tables for other datasets, potentially from S3DIS/Matterport/Scannet200/Scannet++}

% \subsection{Joint 2D - 3D Training}



% \subsection{Downstream Application}





% \clearpage


% \section{Ablations}



% \todo{Let's not use the word panet, rather 3d fusion transformer}

% \adam{add qualitative results}

\subsection{Limitations}

Our experiments reveal the following limitations for \model{}: First, \model{} as well as other SOTA 3D models have sharp decrease in performance when they take sensor point cloud as input instead of the mesh point cloud. This is due to noise in depth and camera poses, resulting in misalignments between RGB-D and mesh. In our future work, we aim to explore inferring depth and camera poses as part of the inference process. Second, the project's focus on investigating a unified architecture leveraging pre-trained features with both 2D and 3D data confines our experiments to small-scale datasets. Future efforts will involve scaling the model through training on diverse 2D and 3D datasets, incorporating free-flowing language and conducting comparisons with state-of-the-art open-vocabulary 3D models in a zero-shot setup.


%underperforms SOTA models . This is in part due to noise in depths, camera poses leading to misalignments between RGB-D and mesh. This limitation is also shared by other SOTA models, as demonstrated  by their sharp decrease in performance when using sensor poincloud as input. In our future work, we aim to explore inferring depth and camera poses as part of the inference process. 



% 1. Sensitivity to depth holes and noise
% 2. Sensitivity to pose errors. 
% These are shared by other point cloud models. 

% Our future directions will explore  inferring depth and camera poses as part of the 3d inference process. 

% this was just a first step to show that these kinds of architectures can work as well and even better than sota 3d specific model. another crucial next step is to scale up training jointly on more 2d and 3d datasets, and study open-vocabulary capabilities in 3d that the model can pick up from diverse datasets in 2D and compare against models that do post-hoc processing over 2d features like openscene. 


% we notice that perception significantly improves as we add more views, but maybe there are scenarios where we can't afford to have a ton of views. potentially generative models can utilize their priors to do completion in 3d and let us operate with less views



%A 3D perceoption model should
% \subsection{Maybe Experiments}:
% \begin{itemize}
%     \item Out of domain generalization
%     \item Training jointly on multiple 3D datasets
% \end{itemize}

==> 4_exp_katef.tex <==
\section{Experiments}



% Our experiments aim to answer the following questions:
% \begin{enumerate}
% \item How does \model{} compare against the current state-of-the-art in 3D point cloud perception that consumes directly 3D colored point clouds without considering the input RGB-D  images, in established real-world and simulation 3D perception benchmarks? How much do the misalignments between the sensor and mesh obtained point cloud affects performance of \model{} and baselines?
% \item Can \model{} assist perception of embodied agents~\cite{helper} that move around in dynamic home environments and do not afford a mesh 3D map building stage?
% \item  How much if at all training \model{} across both 2D and 3D visual understanding tasks helps each one of them?
% \item How much  \model{}'s  alternating between 2D and 3D featurization helps over a more straight forward architecture of first within-view and then cross-view feature fusion?
% \item How does \model{}'s performance varies across  2D backbone pre-training? 
% \end{enumerate} 



\subsection{Evaluation on  3D benchmarks}
% \todo{Add open vocabulary works}
\input{tables/real_in_domain_3d}

\paragraph{Datasets:} First, we test our model in   instance and semantic 3D segmentation in   ScanNet~\cite{scannet} and ScanNet200~\cite{scannet200} benchmarks. The objective in these benchmarks is to label the point cloud sampled from the 3D mesh of a scene reconstructed from raw sensor data. ScanNet uses 20  common semantic classes  and ScanNet200 uses 200 classes with varying amount of representation in the dataset. As a result, ScanNet200 is more representative of the long-tailed object distribution encountered in the real world. 

\paragraph{Evaluation metrics:} We follow the standard evaluation metrics, namely mean Average Precision (mAP) for instance segmentation and mean Intersection over Union (mIoU) for semantic segmentation.

\paragraph{Baselines:}
We compare our model against several 3d point cloud models that directly take the mesh-sampled 3D point cloud as input~\cite{} which we have already discussed in related work. 
We also consider 
%Mask3D is the current SOTA in ScanneT

consider the following baselines:
1. Mask3D~\cite{}


Existing SOTA methods directly feed the mesh-sampled 3D point cloud to their model. 
However, many applications require direct processing of the raw data without going through an expensive mesh creation process. Moreover, as motivated before, utilizing RGB-D input can enable us to more closely unify 2D and 3D perception and benefit from pre-trained features and abundant 2D data. Motivated by this, we benchmark state-of-the-art 3D models in the setup where the input to their model is a point cloud obtained by directly unprojecting the posed RGB-D images. 
%We also compare all models in the original setup where mesh point clouds are available. 

\nikos{why do we need this?} We also compare with OpenMask3D~\cite{openmask3d}, a state-of-the-art zero-shot 3D instance segmentation model using CLIP~\cite{clip} 2D features. Note that our approach is fully supervised, making the comparison unfair, but we include it for completeness.

We also compare with OpenScene~\cite{openscene}, a state-of-the-art zero-shot 3D semantic segmentation model that uses 2D features from LSeg~\cite{lseg} and OpenSeg~\cite{openseg}. This is a zero-shot method in contrast to fully-supervised approach to ours, thus making the comparison unfair, but we include it for completeness.

We also compare with OpenScene~\cite{openscene}, a state-of-the-art zero-shot 3D semantic segmentation model that uses 2D features from LSeg~\cite{lseg} and OpenSeg~\cite{openseg}. This is a zero-shot method in contrast to fully-supervised approach to ours, thus making the comparison unfair, but we include it for completeness.


our model outperforms all methods operating over sensor RGB point cloud including the recent Deep View Aggregation~\cite{deepview}. Additionally, our model closely matches the performance of the Virtual Multiview Fusion method~\cite{virtualview}, which generates RGB-D images from the provided mesh, incorporates design heuristics for camera view sampling to avoid occlusions, ensures balanced scene coverage, and employs higher field-of-views.$^\dagger$ \let\thefootnote\relax\footnotetext{$^{\dagger}$their code/data is not publicly available}


\paragraph{Settings:}
We consider the following settings for point cloud models:

1. Mesh-sampled point cloud:

2. Rendered point cloud: 

3. Sensor point cloud:








%We first compare our model with state-of-the-art 3D models in popular established benchmarks of ScanNet~\cite{scannet} and Scannet200~\cite{scannet200} for instance and semantic segmentation tasks in Tables-\ref{tab:established_3d}. In these benchmarks, the task is to label the point cloud sampled from the mesh of a scene reconstructed from the raw sensor data. 

shoudl We show results for our model and baselines  in Tables-\ref{tab:established_3d}. We draw the following conclusions:
% We draw the following conclusions: 

% \begin{itemize}
\textbf{1. Our model is 10\% and 6\% behind the 3D mesh SOTA methods in mAP and mAP50,  but matches them in mAP25} This is due to misalignments between camera poses and the extracted 3D mesh, that in tight  scoring thresholds matters more.


%\textbf{1. Performance of 3D point cloud models drops with sensor point cloud as input.} (Table~\ref{tab:scannet_ins}): SOTA Mask3D's performance drops from 55.2\% mAP with mesh point cloud input to 43.9\% mAP with sensor point cloud input. This is consistent with prior works~\cite{virtualview,deepview} in 3D semantic segmentation on ScanNet, which attributes the drop to misalignments caused by noise in camera poses, depth variations and post-processing steps.

\textbf{2. \model{} outperforms SOTA 3D methods with sensor point cloud input} (Table~\ref{tab:scannet_ins}): Performance of 3D point cloud models significantly drops with sensor point cloud as input! SOTA Mask3D's performance drops from 55.2\% mAP with mesh point cloud input to 43.9\% mAP with sensor point cloud input. This is consistent with prior works~\cite{virtualview,deepview} in 3D semantic segmentation on ScanNet, which attributes the drop to misalignments caused by noise in camera poses, depth variations and post-processing steps.

%Our model with Swin-Base (Swin-B) backbone significantly outperforms SOTA Mask3D model with sensor point cloud input by 4.1\%, 9.2\% and 13.6\% in mAP, mAP50 and mAP25 respectively. Our model achieves comparable performance to methods using mesh-sampled point cloud input, particularly on the mAP25 metric.
    
\textbf{3. \model{} sets a new SOTA in semantic segmentation on ScanNet} (Table~\ref{tab:scannet_sem}). It outperforms 3D point cloud methods and other methods that featurize images. 

%Notably, our model also closely matches SOTA methods utilizing mesh-sampled point cloud. %\nikos{why do we need this?} 
    
\textbf{4. \model{} sets a new instance segmentation SOTA on the long-tailed ScanNet200 dataset} (Table~\ref{tab:scannet200_ins}) while exclusively utilizing sensor RGB-D data. his highlights the contribution of 2D features, particularly in detecting a long tail of class distribution where limited 3D data is available. We show more detailed results with performance on the head, common and tail classes in supplementary. \todo{We should indeed check if the major gains are in the long tail classes}

%: our model outperforms SOTA Mask3D with sensor point cloud input by 14.5\% mAP. It also outperforms SOTA mesh-point-cloud-based methods including very recent works of QueryFormer~\cite{queryformer} and MAFT~\cite{maft} by 0.8\% mAP, 4.8\% mAP50 and 7.6\% mAP25 establishing a new SOTA on this benchmark while exclusively utilizing sensor RGB-D data. This highlights the contribution of 2D features, particularly in detecting a long tail of class distribution where limited 3D data is available. We show more detailed results with performance on the head, common and tail classes in supplementary. 

\textbf{5. \model{} sets a new semantic segmentation SOTA on ScanNet200} (Table~\ref{tab:scannet200_sem}), outperforming SOTA semantic segmentation models that use mesh point clouds by 5.6\%.
    
  %  \todo{We should indeed check if the major gains are in the long tail classes}
    
    %We observe that our model outperforms SOTA Mask3D in the sensor point cloud setup by X\% and even outperforms the models trained on mesh point cloud by Y\%, thus setting a new state-of-the-art in this benchmark. This indicates that 2D features can significantly help when tasked with detecting a long-tail of class distribution where we do not possess a lot of 3D data.
% \end{itemize}

% \todo{CAUTION: GARBAGE Ahead!}
\input{tables/ai2thor}

\subsection{Evaluation on multiview RGB-D in simulation}
As highlighted earlier, misalignments between sensor RGB-D and mesh-sampled point clouds can significantly impact performance. Conventional 3D datasets, such as ScanNet~\cite{scannet, scannet200}, annotate the 3D mesh directly and project annotations onto sensor RGB-D images. However, these RGB-D labels inherit misalignment issues and noise due to the sparser mesh compared to RGB-D images, thus making them unsuitable for training and evaluation. To overcome this, we collect RGB-D data in the popular Ai2Thor~\cite{ai2thor} embodied simulation environment using procedural homes generated by ProcThor~\cite{procthor}. Our dataset comprises 1500 scenes, divided into 1200 training and 300 test scenes to maintain a dataset size comparable to ScanNet~\cite{scannet}. By randomly placing a robot agent at navigable locations from the simulator, we record RGB-D and camera information, facilitating the study of perception in RGB-D setups without misalignment issues.

We train and evaluate our model and SOTA Mask3D~\cite{mask3d} on the unprojected RGB-D images. As shown in Table-\ref{tab:sim}, our model outperforms Mask3D by 7\% mAP, showing strong performance in a directly comparable RGB-D setup. Despite the 2D features being pre-trained on real-world data, traditionally considered less beneficial in simulated environments, our architecture leverages pre-trained features effectively. This improvement underscores the potential of unified 2D-3D architectures in enhancing 3D perception. It suggests that current real-world benchmarks may restrain these models due to misalignments. We hope this encourages the community to also focus on directly collecting, labeling, and benchmarking RGB-D sensor data. %In supplementary, we show that we improve performance on categories common with ScanNet dataset as well

%As highlighted in the previous section, the misalignments between the sensor RGB-D and mesh sampled point cloud can result in a sharp decrease in performance. Most popular real-world 3D datasets annotate the 3D mesh directly and project these annotations to the sensor RGB-D images. However, these RGB-D labels inherit the misalignment issues and additionally have noises due to the mesh being much sparser than the RGB-D images making them unsuitable for training and benchmarking on their RGB-D data. Thus, to study perception in RGB-D setup directly independent of the misalignment issues, we generate a scannet scale data of 1300 train scenes and 300 validation scenes from ProcThor~\cite{procthor} which is based on Ai2Thor~\cite{ai2thor} a popular simulation environment in embodied AI community. We spawn a robot agent randomly at the simulator provided navigable locations and record the RGB-D information and camera information.

%We train and evaluate our model and SOTA Mask3D on the unprojected RGB-D images. We observe that our model outperforms Mask3D by 7\% mAP showing strong performance in a comparable RGB-D setup. 

\subsection{3D perception for embodied agents in simulation}
\input{tables/teach}
% \todo{NEEDS REFINEMENT} \\

\input{tables/joint_2d_3d}
\input{tables/ablations_alt}
% \todo{also explain, seen and unsene splits of these datasets, and motivate that mesh reconstruction is not really possible or practical}
We apply our model in embodied setups (TEACh~\cite{teach} and Alfred~\cite{alfred}) in a setup where agents have depth and camera poses. In TEACh's Trajectory from Dialogue (TfD) setup, agents follow dialogues to perform tasks, while in Alfred they execute high/low-level instructions. A critical component for successful execution is object detection. Prior SOTA embodied methods~\cite{helper,film} use single-view object detectors and heuristic-based object trackers to link 2D instances into a 3D semantic map. We replace these with \model{} trained for instance segmentation on the training set of TEACh~\cite{teach}, processing the last 10  egocentric views of the agent trajectory and adding the predicted instances to the 3D semantic map of HELPER~\cite{helper}. We use Task Success Rate (SR) to assess if the agent completes the entire task and Goal Conditioned Success Rate (GC) to evaluate the proportion of goal conditions satisfied across all episodes following standard evaluation protocols~\cite{alfred, teach}. Evaluation is performed on both "valid-seen" (similar to the training set) and "valid-unseen" (different houses) splits. In Table-\ref{tab:embodied}, we observe that using \model{} significantly boosts SOTA success rate of HELPER by 2.8\% in the unseen validation split TEACh and by 10.3\% in Alfred's unseen validation split. 

%processing multiple views directly for 3D instance segmentation. We utilize \model{} on the last 10 egocentric views of the agent trajectory to obtain object instances. 


%We study an application of our perception model in the embodied setup of TEACh~\cite{teach} and Alfred~\cite{alfred} in the setup where agents have access to depth and camera poses from the simulator. We evaluate on the Trajectory From Dialogue (TfD) setup of TEACh, where the agent follows a dialogue between two human annotators to complete a given task in an embodied environment like ``Make a sandwich". The Alfred benchmark similarly evaluates the agent's ability to carry out high-level (“Rinse off a mug and place it in the coffee maker”) and low-level (“Walk to the coffee maker on the right”) instructions provided by a user. A critical component for successful execution is object detection. Prior SOTA methods on TEACh like HELPER~\cite{helper} use single-view object detectors to detect objects and a heuristic-based object tracker to link instances of a particular object to build a 3D semantic map of the scene. Since, the agent is inherently embodied and naturally has access to multiple views, we replace the single-view object detector and tracker from HELPER with \model{}, which can process multiple views and directly produce instance segmentations in 3D.
%Specifically, we run \model{} on the last 10 egocentric views of the agent trajectory to obtain a set of object instances based on multiple viewpoints. These instances are added to the 3D semantic map of the scene to be used for object navigation and interaction necessary to carry out the instruction following Helper~\cite{helper}. 
%\textbf{Evaluation Metrics} Following standard evaluation protocols~\cite{alfred, teach}, we employ the following metrics a) \textit{Task success rate (SR)} which evaluates if the agent successfully completed the entire task. b) \textit{Goal Conditioned Success Rate (GC)} which evaluates the proportion of goal conditioned achieved across all episodes. We evaluate all models on ``valid-seen" and ``valid-unseen" splits, where valid-seen comprises houses similar in distribution to train set, while ``valid-unseen" have different houses. 
%In Table-\ref{tab:embodied}, we compare Helper~\cite{helper} with \model{} as its perception system as a replacement to its single-view object detector and heuristic-based tracker. Using \model{} significantly boosts SOTA success rate of Helper by 2.8\% in the unseen validation split TEACh and by 10.3\% in Alfred's unseen validation split. 

% \todo{gabe; what do we do specifically? how many images do we process? how do we handle dynamic objects? any other useful detail?}

%\textbf{Evaluation Metrics} Following standard evaluation protocols~\cite{alfred, teach}, we employ the following metrics a) \textit{Task success rate (SR)} which evaluates if the agent successfully completed the entire task. b) \textit{Goal Conditioned Success Rate (GC)} which evaluates the proportion of goal conditioned achieved across all episodes. %Additionally, we provide path-length-weighted variants, where the weights are determined by the ratio of the expert trajectory's path length to the agent's taken path length.







\subsection{Joint 2D-3D Training}

% \todo{needs refinement}
\model{} is designed to generate segmentation masks for both single 2D RGB images and multiview RGB-D image sequences, while sharing the majority of parameters. Table~\ref{tab:joint} shows results when jointly training with 3D data from ScanNet~\cite{scannet} and 2D data from COCO~\cite{coco}. %We interleave 2D and 3D batches during training. 
We compare our model to a variant trained independently on 2D or 3D data. We find that joint training yields a 2.6\% improvement in 3D, accompanied by a slight drop in 2D. While training the model we observe that the performance on COCO continues to improve, whereas on ScanNet it starts to decline much earlier. This highlights the need to explore smarter strategies for balancing 2D and 3D data during training to prevent overfitting to one domain over the other.








%We notice that \model{} on COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other.

%Note that the 3D \model{} trained on Scannet only (in row 3) starts from pre-trained weights from Mask2Former~\cite{m2f} trained on COCO. The additional boost with joint-training suggests that it can improve performance in 3D by helping the model not to overfit on the 3D RGB-D images. We notice that COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other. Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.


%Given the higher resolution of COCO images (1024 X 1024) compared to Scannet images (256 X 256), we randomly downsample COCO images to 256 X 256 for data augmentation, aligning the 2D and 3D image resolutions. 
%We compare our model to our model's variant trained independently on 2D and 3D data. We find that joint training yields a 1.4\% improvement in 3D performance, accompanied by a slight drop in 2D performance. Note that the 3D \model{} trained on Scannet only (in row 3) starts from pre-trained weights from Mask2Former~\cite{m2f} trained on COCO. The additional boost with joint-training suggests that it can improve performance in 3D by helping the model not to overfit on the 3D RGB-D images. We notice that COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other. Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time. %We show Odin's performance when we take the best checkpoint in individual domain. 

%Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.

%This suggests that joint training 3D models with 2D data can improve performance even . Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.


%We design our architecture to handle both 2D and 3D data while sharing majority of the parameters. In this section, we train our model jointly on 3D data from scannet and 2D dataset from COCO. During training, we interleave sampling batches from 2D and 3D data. Since the images in COCO are at higher resolution of 1024 X 1024, while the scannet images are at 256 X 256 resolution, we randomly downsample COCO images to 256 X 256 as a data augmentation to match the 2D and 3D image resolutions. We compare our model against a variant of our model trained independently on 2D and the 3D data. We find that joint training helps 3D performance by 1.4\% while incurring slight performance drop in 2D. This indicates that jointly training 3D models with 2D data can help fight overfitting and improve validation performance. More importantly, we have a single unified model that, at test time, can produce segmentation masks over either single 2D RGB image or multiview RGB-D images. 
% Analysis:
% 1) sim versus real-> inaccuracy of poses
% 2) sensed mesh versus given mesh:huge difference in the numbers
% 3) long tail discussion!
% 4) virtual views: 


\subsection{Ablations}
% \input{tables/ablations}


\textbf{Cross-View fusion is crucial for instance segmentation but not for semantic segmentation} (Table~\ref{tab:cross_view}): removing cross-view contextualization layers results in a 6.9\% mAP drop for instance segmentation, while only causing a 1.3\% mIoU drop in semantic segmentation. \todo{ Recent 3D open-vocabulary works \todo{???!!!}~\cite{conceptfusion,openscene} without strong cross-view fusion only focus on semantic segmentation and thus could not uncover this issue.}

\textbf{Interleaving within-view and cross-view fusion helps. } (Table~\ref{tab:where_cross}): row-2 shows a 5.7\% mAP drop when cross-view fusion happens after the image is processed using the full backbone instead of interleaving the within-view and cross-view fusion. Our finding aligns with the observation from Deep View Aggregation~\cite{deepview} that early fusion is beneficial. 

%Moreover, performing fusion only in the backbone, excluding upsampling layers, results in a 2\% performance drop (row-3), highlighting the importance of additional fusion layers to maintain feature consistency across views after 2D operations.

\textbf{2D weight re-training helps.} (Table~\ref{tab:pretrain}): initializing only the image backbone with pre-trained weights, instead of using all shared layers, results in a 4.7\% mAP drop (row-2). Starting the entire model from scratch leads to a larger drop of 9.1\% mAP (row-3). This underscores the importance of sharing as many parameters as possible with the 2D models to leverage their pre-trained weights effectively.

\textbf{Higher capacity 2D backbone helps}

\textbf{Finetuning 2D backbone helps
increases performance (Table~\ref{tab:backbone_frozen}): using Swin-B over ResNet-50 leads to performance gains, suggesting that \model{} can directly benefit from advancements in 2D computer vision. However, this gain is not obvious when the backbone is frozen. Specifically, freezing the ResNet-50 backbone shows similar mAP performance with a 0.6\% mIoU drop, while for Swin, freezing results in a 2.4\% mAP drop and 1.3\% mIoU drop. Intuitively, unfreezing the backbone allows 2D layers to adapt to cross-view fused features better and Swin-B benefits more from this adaptation. Therefore, we keep our backbone unfrozen in all experiments.

\textbf{Supplying 2D features directly to 3D models provides no benefit} (Table~\ref{tab:mask3d_2d}): incorporating 2D features alongside XYZ+RGB in Mask3D yields performance comparable to a model lacking access to 2D features.

%We unproject 2D features from Resnet-50 and supply it as an additional input to Mask3D. We find that it results in a marginal increase in task performance. Thus, while always using 2D features might be a good idea, directly supplying these features to a 3D backbone might not be an optimal design as also shown by our 2nd ablation bullet. 

% \todo{Mention DBSCAN}

% \todo{1. no alternating. sharing weights and alternating 2d 3d, do we have this number?}
% \todo{2. no cross view fusion}
% \todo{joint 2d 3d}
% \todo{many 3d}
% \todo{2d backbone variation}
% \todo{no 2d pretraining}
% \todo{straightforward addition of 2d feats to mask3d}

% \subsection{zero shot??}





% \todo{make sure we bold numbers on tables}
% \begin{table}
% \caption{\textbf{Comparison on Scannet for Instance Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llccccc}

% Input & Model & mAP &  mAP50 & mAP25 \\ \hline
% \multirow{4}{*}{Sensor RGBD point cloud} & Mask3D $^{\dagger}$ & 43.9 & 60.0 & 69.9  \\
%  & Ours-Resnet50 & 45.7 & 66.3  & 81.8  \\
%  % & Ours-Swin-T &  &  &   \\
%  & Ours-Swin-L & 48.0 & 69.2 & 83.5  \\ \hline
% \multirow{2}{*}{Mesh Sampled point cloud} & SoftGroup & 46.0 & 67.6 & 78.9 \\
% & Mask3D & 55.2 & 73.7 & 83.5 \\
%  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table}
% \caption{\textbf{Comparison on Scannet for Semantic Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llc} 
% Input & Model & mIoU \\ \hline
% \multirow{8}{*}{Sensor RGBD point cloud} 
% & MVPNet & 68.3\\
% & BPNet & 69.7 \\
% & DeepViewAgg & 71.0 \\
%  & Ours-Resnet50 & 73.2  \\
%  % & Ours-Swin-T &    \\
%  & Ours-Swin-L & 76.0 \\ \hline
% \multirow{2}{*}{Rendered RGBD point cloud} & VMVF & 76.4 \\
% & Ours & \\ \hline
% \multirow{2}{*}{Mesh Sampled point cloud} & Point Transformer v2 & 75.4 \\
% & Swin3D-L & 76.7  \\
%  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table*}
% \caption{\textbf{Comparison on Scannet200 for Instance Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{llcccccccccccc}

% Input & Model & \multicolumn{3}{c}{All} &  \multicolumn{3}{c}{Head} & \multicolumn{3}{c}{Common} & \multicolumn{3}{c}{Tail} \\
%  \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}  
% & & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25\\ \midrule
% \multirow{3}{*}{Sensor RGBD point cloud} & Mask3D $^{\dagger}$ & 15.5 & 21.4 & 24.3 & 21.9 & 31.4 &  37.1 & 13.0 & 17.2 & 18.9 & 7.9 & 10.3 & 11.5 \\
%  & Ours-Resnet50 & 26.0 & 37.6 & 43.8 &  &  &  &  &  &  &  &  &  \\
%  % & Ours-Swin-T &  &  &   \\
%  & Ours-Swin-L (in progress) &     &         &   &  & & &   \\ \midrule
% \multirow{1}{*}{Mesh Sampled point cloud} & Mask3D & 27.4 & 37.0  & 42.3 \\
%  \midrule
% \end{tabular}
% }
% \end{table*}


% \begin{table}
% \caption{\textbf{Comparison on Scannet200 for Instance Segmentation Task}}

% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llccc}

% Input & Model  & mAP &  mAP50 & mAP25 \\ \midrule
% \multirow{3}{*}{Sensor RGBD point cloud} & Mask3D $^{\dagger}$ & 15.5 & 21.4 & 24.3  \\
%  & Ours-Resnet50 & 26.0 & 37.6 & 43.8  \\
%  & Ours-Swin-L &  30.0        &  43.0         &  51.0   \\ \midrule
% \multirow{1}{*}{Mesh Sampled point cloud} & Mask3D & 27.4 & 37.0  & 42.3 \\
%  \midrule
% \end{tabular}
% }
% \end{table}





% \todo{Maybe tables for other datasets, potentially from S3DIS/Matterport/Scannet200/Scannet++}

% \subsection{Joint 2D - 3D Training}



% \subsection{Downstream Application}





% \clearpage


% \section{Ablations}



% \todo{Let's not use the word panet, rather 3d fusion transformer}

\adam{add qualitative results}

\subsection{Limitations}

Our experiments reveal the following limitations for \model{}: First, \model{} as well as other SOTA 3D models have sharp decrease in performance when they take sensor point cloud as input instead of the mesh point cloud. This is due to noise in depth and camera poses, resulting in misalignments between RGB-D and mesh. In our future work, we aim to explore inferring depth and camera poses as part of the inference process. Second, the project's focus on investigating a unified architecture leveraging pre-trained features with both 2D and 3D data confines our experiments to small-scale datasets. Future efforts will involve scaling the model through training on diverse 2D and 3D datasets, incorporating free-flowing language and conducting comparisons with state-of-the-art open-vocabulary 3D models in a zero-shot setup.


%underperforms SOTA models . This is in part due to noise in depths, camera poses leading to misalignments between RGB-D and mesh. This limitation is also shared by other SOTA models, as demonstrated  by their sharp decrease in performance when using sensor poincloud as input. In our future work, we aim to explore inferring depth and camera poses as part of the inference process. 



% 1. Sensitivity to depth holes and noise
% 2. Sensitivity to pose errors. 
% These are shared by other point cloud models. 

% Our future directions will explore  inferring depth and camera poses as part of the 3d inference process. 

% this was just a first step to show that these kinds of architectures can work as well and even better than sota 3d specific model. another crucial next step is to scale up training jointly on more 2d and 3d datasets, and study open-vocabulary capabilities in 3d that the model can pick up from diverse datasets in 2D and compare against models that do post-hoc processing over 2d features like openscene. 


% we notice that perception significantly improves as we add more views, but maybe there are scenarios where we can't afford to have a ton of views. potentially generative models can utilize their priors to do completion in 3d and let us operate with less views



%A 3D perceoption model should
% \subsection{Maybe Experiments}:
% \begin{itemize}
%     \item Out of domain generalization
%     \item Training jointly on multiple 3D datasets
% \end{itemize}

==> 4_experiments_old.tex <==
\section{Experiments}

\subsection{Evaluation on  3D benchmarks}
% \todo{Add open vocabulary works}
\input{tables/real_in_domain_3d}
\noindent \textbf{Datasets:} First, we test our model in   instance and semantic 3D segmentation in   ScanNet~\cite{scannet} and ScanNet200~\cite{scannet200} benchmarks. The objective in these benchmarks is to label the point cloud sampled from the 3D mesh of a scene reconstructed from raw sensor data. ScanNet evaluates on 20 common semantic classes, while ScanNet200 uses 200 classes, providing a more representative representation of the long-tailed object distribution encountered in the real world. We report results on the official validation split of these datasets.

\noindent \textbf{Evaluation metrics:} We follow the standard evaluation metrics, namely mean Average Precision (mAP) for instance segmentation and mean Intersection over Union (mIoU) for semantic segmentation.

\noindent \textbf{Baselines:} In \textit{instance segmentation}, our main baseline is SOTA 3D method Mask3D~\cite{mask3d}. We also compare with recent and concurrent work to ours of PBNet~\cite{pbnet}, QueryFormer~\cite{queryformer} and MAFT~\cite{maft}. QueryFormer and MAFT improve the query initialization and refinement in Mask3D-like architecture and thus have complementary advantages to ours. Unlike \model{}, these methods directly process point clouds and start training all their weights from scratch.
 As motivated before, utilizing RGB-D input directly has several advantages, including avoiding costly mesh building processes, achieving closer integration of 2D and 3D perception, and leveraging pre-trained features and abundant 2D data. Thus, we train both SOTA Mask3D and our model with sensor RGB-D point cloud input, consistently evaluating all methods on benchmark-provided mesh-sampled point clouds. 
%Moreover, as motivated before, utilizing RGB-D input directly can enable us to avoid costly mesh building processes, more closely unify 2D and 3D perception and benefit from pre-trained features and abundant 2D data. We evaluate both SOTA Mask3D and our model by training them with sensor RGB-D point cloud input while still labeling the benchmark mesh-sampled point cloud.
For \textit{semantic segmentation}, we compare with MVPNet~\cite{mvpnet}, BPNet~\cite{bpnet} and state-of-the-art DeepViewAgg~\cite{deepview} which directly operate on sensor RGB images and point clouds. We also compare with VMVF~\cite{virtualview} which operate over rendered RGB-D images from the provided mesh, with heuristics for camera view sampling to avoid occlusions, ensures balanced scene coverage, and employs higher field-of-views$^\dagger$ \let\thefootnote\relax\footnotetext{$^{\dagger}$their code/data is not publicly available}. Similar to \model{}, all these methods utilize 2D pre-trained backbones. We also compare with Point-Transformer v2 \cite{ptv2}, Stratified Transformer \cite{stratified}, OctFormer \cite{octformer} and Swin3D-L \cite{swin3d} that process the mesh-sampled point cloud directly, without using any 2D pre-training.  In ScanNet200 semantic segmentation benchmark, we compare with SOTA OctFormer \cite{octformer} and with CeCo~\cite{ceco}, a baseline especially designed to fight class-imbalance in ScanNet200. These methods directly process the point cloud and do not use 2D pre-trained weights. We also compare with LGround \cite{scannet200} which uses 2D CLIP pre-training. We also compare with zero-shot 2D foundation model-based 3D models of OpenScene~\cite{openscene} and OpenMask3D~\cite{openmask3d}. This comparison is unfair since they are not supervised within domain, but we include them for completeness.


%We compare our model against several 3d point cloud models that directly take the mesh-sampled 3D point cloud as input~\cite{mask3d} which we have already discussed in related work. 

%First, we benchmark our model against state-of-the-art 3D models on  ScanNet~\cite{scannet} and Scannet200~\cite{scannet200}, both for instance and semantic segmentation. The objective in these benchmarks is to label the point cloud sampled from the mesh of a scene reconstructed from raw sensor data. ScanNet200 extends ScanNet by benchmarking on 200 classes with a long-tail distribution instead of the 20 common classes used in ScanNet. Most SOTA methods directly feed the mesh-sampled point cloud to their model. However, many applications require direct processing of the raw data without going through an expensive mesh creation process. Moreover, as motivated before, utilizing RGB-D input can enable us to more closely unify 2D and 3D perception and benefit from pre-trained features and abundant 2D data. Motivated by this, we benchmark state-of-the-art 3D models in the setup where the input to their model is a point cloud obtained by directly unprojecting the raw sensor data. We also compare all models in the original setup where mesh point clouds are available. 

%\paragraph{Evaluation metrics:} We follow the standard evaluation metrics, namely mean Average Precision (mAP) for instance segmentation and mean Intersection over Union (mIoU) for semantic segmentation.






%We first compare our model with state-of-the-art 3D models in popular established benchmarks of ScanNet~\cite{scannet} and Scannet200~\cite{scannet200} for instance and semantic segmentation tasks in Tables-\ref{tab:established_3d}. In these benchmarks, the task is to label the point cloud sampled from the mesh of a scene reconstructed from the raw sensor data. 
The results are presented in \cref{tab:established_3d}. 
We draw the following conclusions: 

% \begin{itemize}

\noindent \textbf{Performance drops with sensor point cloud as input} (\cref{tab:scannet_ins}): SOTA Mask3D's performance drops from 55.2\% mAP with mesh point cloud input to 43.9\% mAP with sensor point cloud input. This is consistent with prior works~\cite{virtualview,deepview} in 3D semantic segmentation on ScanNet, which attributes the drop to misalignments caused by noise in camera poses, depth variations and post-processing steps.

\noindent \textbf{\model{} outperforms SOTA 3D methods with sensor point cloud input} (\cref{tab:scannet_ins}): Our model significantly outperforms SOTA Mask3D model with sensor point cloud input and achieves comparable performance to methods using mesh-sampled point cloud input on the mAP25 metric.
    
\noindent \textbf{\model{} sets a new SOTA in sensor-based semantic segmentation on ScanNet} (\cref{tab:scannet_sem}): outperforming all methods operating over sensor RGB point cloud including the SOTA DeepViewAgg~\cite{deepview}. Additionally, our model closely matches the performance of models operating on rendered RGB-D point cloud and mesh sampled point cloud. 
%the Virtual Multiview Fusion method~\cite{virtualview}, which generates RGB-D images from the provided mesh, incorporates design heuristics for camera view sampling to avoid occlusions, ensures balanced scene coverage, and employs higher field-of-views.$^\dagger$ \let\thefootnote\relax\footnotetext{$^{\dagger}$their code/data is not publicly available} 
%Notably, our model also closely matches SOTA methods utilizing mesh-sampled point cloud. \nikos{why do we need this?} We also compare with OpenScene~\cite{openscene}, a state-of-the-art zero-shot 3D semantic segmentation model that uses 2D features from LSeg~\cite{lseg} and OpenSeg~\cite{openseg}. This is a zero-shot method in contrast to fully-supervised approach to ours, thus making the comparison unfair, but we include it for completeness.

\noindent \textbf{\model{} sets a new instance segmentation SOTA on the long-tailed ScanNet200 dataset} (\cref{tab:scannet200_ins}): outperforming SOTA 3D models on all setups including the models trained on mesh-sampled point cloud, thus establishing a new SOTA on this benchmark while exclusively utilizing sensor RGB-D data. This highlights the contribution of 2D features, particularly in detecting a long tail of class distribution where limited 3D data is available. We show more detailed results with performance on the head, common and tail classes in supplementary.

%our model outperforms SOTA Mask3D with sensor point cloud input by 14.5\% m%AP. It also outperforms SOTA mesh-point-cloud-based methods, establishing a new SOTA on this benchmark while exclusively utilizing sensor RGB-D data. This highlights the contribution of 2D features, particularly in detecting a long tail of class distribution where limited 3D data is available. We show more detailed results with performance on the head, common and tail classes in supplementary. %\nikos{why do we need this?} We also compare with OpenMask3D~\cite{openmask3d}, a state-of-the-art zero-shot 3D instance segmentation model using CLIP~\cite{clip} 2D features. Note that our approach is fully supervised, making the comparison unfair, but we include it for completeness.

\noindent \textbf{\model{} sets a new semantic segmentation SOTA on ScanNet200} (\cref{tab:scannet200_sem}), outperforming SOTA semantic segmentation models that use mesh point clouds.
    
    % \todo{We should indeed check if the major gains are in the long tail classes}
    
    %We observe that our model outperforms SOTA Mask3D in the sensor point cloud setup by X\% and even outperforms the models trained on mesh point cloud by Y\%, thus setting a new state-of-the-art in this benchmark. This indicates that 2D features can significantly help when tasked with detecting a long-tail of class distribution where we do not possess a lot of 3D data.
% \end{itemize}

% \todo{CAUTION: GARBAGE Ahead!}
\input{tables/ai2thor}

\subsection{Evaluation on multiview RGB-D in simulation}
Using the Ai2Thor~\cite{ai2thor} simulation environment with procedural homes from ProcThor~\cite{procthor}, we collected RGB-D data for 1500 scenes (1200 training, 300 test) of similar size as ScanNet.
%As highlighted earlier, misalignments between sensor RGB-D and mesh-sampled point clouds can significantly impact performance. Conventional 3D datasets, such as ScanNet~\cite{scannet, scannet200}, annotate the 3D mesh directly and project annotations onto sensor RGB-D images. However, these RGB-D labels inherit misalignment issues and noise due to the sparser mesh compared to RGB-D images, thus making them unsuitable for training and evaluation. To overcome this, we collect RGB-D data in the popular Ai2Thor~\cite{ai2thor} embodied simulation environment using procedural homes generated by ProcThor~\cite{procthor}. Our dataset comprises 1500 scenes, divided into 1200 training and 300 test scenes to maintain a dataset size comparable to ScanNet~\cite{scannet}. By randomly placing a robot agent at navigable locations from the simulator, we record RGB-D and camera information, facilitating the study of perception in RGB-D setups without misalignment issues.
We train and evaluate our model and SOTA Mask3D~\cite{mask3d} on the unprojected RGB-D images. As shown in \cref{tab:sim}, our model outperforms Mask3D by 7\% mAP, showing strong performance in a directly comparable RGB-D setup.
%Despite the 2D features being pre-trained on real-world data, traditionally considered less beneficial in simulated environments, our architecture leverages pre-trained features effectively. This improvement underscores the potential of unified 2D-3D architectures in enhancing 3D perception. 
It suggests that current real-world benchmarks may restrain these models due to misalignments. We hope this encourages the community to also focus on directly collecting, labeling, and benchmarking RGB-D sensor data. %In supplementary, we show that we improve performance on categories common with ScanNet dataset as well

%As highlighted in the previous section, the misalignments between the sensor RGB-D and mesh sampled point cloud can result in a sharp decrease in performance. Most popular real-world 3D datasets annotate the 3D mesh directly and project these annotations to the sensor RGB-D images. However, these RGB-D labels inherit the misalignment issues and additionally have noises due to the mesh being much sparser than the RGB-D images making them unsuitable for training and benchmarking on their RGB-D data. Thus, to study perception in RGB-D setup directly independent of the misalignment issues, we generate a scannet scale data of 1300 train scenes and 300 validation scenes from ProcThor~\cite{procthor} which is based on Ai2Thor~\cite{ai2thor} a popular simulation environment in embodied AI community. We spawn a robot agent randomly at the simulator provided navigable locations and record the RGB-D information and camera information.

%We train and evaluate our model and SOTA Mask3D on the unprojected RGB-D images. We observe that our model outperforms Mask3D by 7\% mAP showing strong performance in a comparable RGB-D setup. 

\subsection{Embodied Instruction Following with \model{}}
\input{tables/teach}
% \todo{NEEDS REFINEMENT} \\
\input{tables/joint_2d_3d}
\input{tables/ablations_alt}

% \todo{also explain, seen and unsene splits of these datasets, and motivate that mesh reconstruction is not really possible or practical}
We apply \model{} in the embodied setups (TEACh~\cite{teach} and ALFRED~\cite{alfred}) where agents have access to RGB, depth and camera poses. These agents operate in dynamic home environments and cannot afford expensive mesh building steps. In TEACh, agents follow dialogues to perform tasks, while in Alfred they execute language instructions. Detecting objects well is critical for task success. Prior SOTA methods~\cite{helper,teach} run per-view 2D instance segmentation models \cite{m2f,solq} and link the detected instances using a simple object tracker. Instead, \model{} processes its last $N$ egocentric views and detect instances directly in 3D. We evaluate using Task Sucess Rate (SR) which checks if the entire task is executed successfully, and Goal Conditioned Success Rate (GC) which checks the proportion of satisfied subgoals across all episodes~\cite{alfred,teach}. We perform evaluation on "valid-seen" (houses similar to the training set) and "valid-unseen" (different houses) splits. In \cref{tab:embodied}, we observe that \model{} with Helper significantly outperforms Helper that uses its original perception pipeline.

%A critical component for successful execution is object detection. Prior SOTA embodied methods~\cite{helper,film} use single-view object detectors and heuristic-based object trackers to link 2D instances into a 3D semantic map. We replace these with \model{} trained for instance segmentation on the training set of TEACh~\cite{teach}, processing the last 10  egocentric views of the agent trajectory and adding the predicted instances to the 3D semantic map of HELPER~\cite{helper}. We use Task Success Rate (SR) to assess if the agent completes the entire task and Goal Conditioned Success Rate (GC) to evaluate the proportion of goal conditions satisfied across all episodes following standard evaluation protocols~\cite{alfred, teach}. Evaluation is performed on both "valid-seen" (similar to the training set) and "valid-unseen" (different houses) splits. In Table-\ref{tab:embodied}, we observe that using \model{} significantly boosts SOTA success rate of HELPER by 2.8\% in the unseen validation split TEACh and by 10.3\% in Alfred's unseen validation split. 

%processing multiple views directly for 3D instance segmentation. We utilize \model{} on the last 10 egocentric views of the agent trajectory to obtain object instances. 


%We study an application of our perception model in the embodied setup of TEACh~\cite{teach} and Alfred~\cite{alfred} in the setup where agents have access to depth and camera poses from the simulator. We evaluate on the Trajectory From Dialogue (TfD) setup of TEACh, where the agent follows a dialogue between two human annotators to complete a given task in an embodied environment like ``Make a sandwich". The Alfred benchmark similarly evaluates the agent's ability to carry out high-level (“Rinse off a mug and place it in the coffee maker”) and low-level (“Walk to the coffee maker on the right”) instructions provided by a user. A critical component for successful execution is object detection. Prior SOTA methods on TEACh like HELPER~\cite{helper} use single-view object detectors to detect objects and a heuristic-based object tracker to link instances of a particular object to build a 3D semantic map of the scene. Since, the agent is inherently embodied and naturally has access to multiple views, we replace the single-view object detector and tracker from HELPER with \model{}, which can process multiple views and directly produce instance segmentations in 3D.
%Specifically, we run \model{} on the last 10 egocentric views of the agent trajectory to obtain a set of object instances based on multiple viewpoints. These instances are added to the 3D semantic map of the scene to be used for object navigation and interaction necessary to carry out the instruction following Helper~\cite{helper}. 
%\textbf{Evaluation Metrics} Following standard evaluation protocols~\cite{alfred, teach}, we employ the following metrics a) \textit{Task success rate (SR)} which evaluates if the agent successfully completed the entire task. b) \textit{Goal Conditioned Success Rate (GC)} which evaluates the proportion of goal conditioned achieved across all episodes. We evaluate all models on ``valid-seen" and ``valid-unseen" splits, where valid-seen comprises houses similar in distribution to train set, while ``valid-unseen" have different houses. 
%In Table-\ref{tab:embodied}, we compare Helper~\cite{helper} with \model{} as its perception system as a replacement to its single-view object detector and heuristic-based tracker. Using \model{} significantly boosts SOTA success rate of Helper by 2.8\% in the unseen validation split TEACh and by 10.3\% in Alfred's unseen validation split. 

% \todo{gabe; what do we do specifically? how many images do we process? how do we handle dynamic objects? any other useful detail?}

%\textbf{Evaluation Metrics} Following standard evaluation protocols~\cite{alfred, teach}, we employ the following metrics a) \textit{Task success rate (SR)} which evaluates if the agent successfully completed the entire task. b) \textit{Goal Conditioned Success Rate (GC)} which evaluates the proportion of goal conditioned achieved across all episodes. %Additionally, we provide path-length-weighted variants, where the weights are determined by the ratio of the expert trajectory's path length to the agent's taken path length.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\columnwidth,keepaspectratio]{figures/qualitative.pdf}
    \caption{\small\textbf{Qualitative Results}} 
    \label{fig:qualitative}
    \vspace{-0.2in}
\end{figure}

\subsection{Joint 2D-3D Training}
We compare joint training of \model{} on sensor RGB-D point cloud from ScanNet dataset and 2D RGB images from COCO dataset to variants trained independently on 2D and 3D data, all initialised  from pre-trained COCO weights. Since there are different classes in ScanNet and COCO, we use our open-vocabulary semantic class-decoding head instead of the vanilla closed-vocabulary head. Results in \cref{tab:joint} show that joint training yields a 2.6\% improvement in 3D, accompanied by a slight drop in 2D. COCO dataset is orders of magnitude bigger than ScanNet, and we observe the model to fit faster on ScanNet, resulting in a scenario where model keeps improving on COCO whereas on ScanNet it starts to decline much earlier. This highlights the need to explore smarter strategies for balancing 2D and 3D data during training to prevent overfitting to one domain over the other --- we leave this for future work. Nevertheless, this experiment highlights the potential benefits of joint training with 2D datasets for 3D segmentation tasks and the benefits of having one architecture for both 2D and 3D parsing tasks. % at test time.






%Thanks to the unified architecture design of \model{}, we experiment with jointly training on 3D ScanNet dataset and 2D COCO dataset and compare it with variants trained independently on 2D and 3D data starting from pre-trained COCO weights as usual. Since there are different classes in ScanNet and COCO, we use our open-vocabulary class-decoding head instead of the vanilla closed-vocabulary head. Results in Table-\ref{tab:joint} show that joint training yields a 2.6\% improvement in 3D, accompanied by a slight drop in 2D. COCO dataset is orders of magnitude bigger than ScanNet, and we observe the model to fit faster on ScanNet, resulting in a scenario where model keeps improving on COCO whereas on ScanNet it starts to decline much earlier. This highlights the need to explore smarter strategies for balancing 2D and 3D data during training to prevent overfitting to one domain over the other --- we leave this for future work.

%Nevertheless, this experiment shows the potential benefit of jointly training with 2D datasets for 3D segmentation tasks and also the possibility of having one architecture that can perform both 2D and 3D tasks at test time. 
% \todo{needs refinement}
%\model{} is designed to generate segmentation masks for both single 2D RGB images and multiview RGB-D image sequences, while sharing the majority of parameters. Table~\ref{tab:joint} shows results when jointly training with 3D data from ScanNet~\cite{scannet} and 2D data from COCO~\cite{coco}. %We interleave 2D and 3D batches during training. 
%We compare our model to a variant trained independently on 2D or 3D data. We find that joint training yields a 2.6\% improvement in 3D, accompanied by a slight drop in 2D. While training the model we observe that the performance on COCO continues to improve, whereas on ScanNet it starts to decline much earlier. This highlights the need to explore smarter strategies for balancing 2D and 3D data during training to prevent overfitting to one domain over the other.







%We notice that \model{} on COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other.

%Note that the 3D \model{} trained on Scannet only (in row 3) starts from pre-trained weights from Mask2Former~\cite{m2f} trained on COCO. The additional boost with joint-training suggests that it can improve performance in 3D by helping the model not to overfit on the 3D RGB-D images. We notice that COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other. Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.


%Given the higher resolution of COCO images (1024 X 1024) compared to Scannet images (256 X 256), we randomly downsample COCO images to 256 X 256 for data augmentation, aligning the 2D and 3D image resolutions. 
%We compare our model to our model's variant trained independently on 2D and 3D data. We find that joint training yields a 1.4\% improvement in 3D performance, accompanied by a slight drop in 2D performance. Note that the 3D \model{} trained on Scannet only (in row 3) starts from pre-trained weights from Mask2Former~\cite{m2f} trained on COCO. The additional boost with joint-training suggests that it can improve performance in 3D by helping the model not to overfit on the 3D RGB-D images. We notice that COCO keeps improving while the scannet performance starts to drop at some point, which means that exploring cleverer strategies of balancing 2D and 3D data during training can ensure that the model does not overfit on one domain before the other. Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time. %We show Odin's performance when we take the best checkpoint in individual domain. 

%Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.

%This suggests that joint training 3D models with 2D data can improve performance even . Importantly, our single unified model can produce segmentation masks for both single 2D RGB images and multiview RGB-D images at test time.


%We design our architecture to handle both 2D and 3D data while sharing majority of the parameters. In this section, we train our model jointly on 3D data from scannet and 2D dataset from COCO. During training, we interleave sampling batches from 2D and 3D data. Since the images in COCO are at higher resolution of 1024 X 1024, while the scannet images are at 256 X 256 resolution, we randomly downsample COCO images to 256 X 256 as a data augmentation to match the 2D and 3D image resolutions. We compare our model against a variant of our model trained independently on 2D and the 3D data. We find that joint training helps 3D performance by 1.4\% while incurring slight performance drop in 2D. This indicates that jointly training 3D models with 2D data can help fight overfitting and improve validation performance. More importantly, we have a single unified model that, at test time, can produce segmentation masks over either single 2D RGB image or multiview RGB-D images. 
% Analysis:
% 1) sim versus real-> inaccuracy of poses
% 2) sensed mesh versus given mesh:huge difference in the numbers
% 3) long tail discussion!
% 4) virtual views: 


\subsection{Ablations}
We conduct our ablation experiments on the ScanNet dataset (\cref{tab:ablations}). Our conclusions are:

\noindent \textbf{Cross-View fusion is crucial for instance segmentation but not for semantic segmentation} (\cref{tab:cross_view}): removing 3D cross-view fusion layers results in a 6.9\% mAP drop for instance segmentation, while a slight drop of 1.3\% mIoU in semantic segmentation. Popular 2D-based 3D open vocabulary works~\cite{conceptfusion,openscene} without strong cross-view fusion only focus on semantic segmentation and thus could not uncover this issue. Row-3 shows a 5.7\% mAP drop when cross-view 3D fusion happens after all within-view 2D layers instead of interleaving the within-view and cross-view fusion. %This aligns with the observation from Deep View Aggregation~\cite{deepview} that early fusion is beneficial.

%\textbf{Interleaving within- and cross-view fusion is important} (Table~\ref{tab:where_cross}): row-2 shows a 5.7\% mAP drop when cross-view fusion happens after the image is processed using the full backbone instead of interleaving the within-view and cross-view fusion. This aligns with the observation from Deep View Aggregation~\cite{deepview} that early fusion is beneficial. Moreover, performing fusion only in the backbone, excluding upsampling layers, results in a 2\% performance drop (row-3), highlighting the importance of additional fusion layers to maintain feature consistency across views after 2D operations.

\noindent \textbf{2D pre-trained weight initialization helps} (\cref{tab:pretrain}): initializing only the image backbone with pre-trained weights, instead of all layers (except the 3D fusion layers), results in a 4.7\% mAP drop (row-2). Starting the entire model from scratch leads to a larger drop of 9.1\% mAP (row-3). This underscores the importance of sharing as many parameters as possible with the 2D models to leverage the maximum possible 2D pre-trained weights.

\noindent \textbf{Stronger 2D backbones helps} (\cref{tab:backbone_frozen}): using Swin-B over ResNet-50 leads to significant performance gains, suggesting that \model{} can directly benefit from advancements in 2D computer vision. 

\noindent \textbf{Finetuning everything including the pre-trained parameters helps} (\cref{tab:backbone_frozen}): while ResNet50's performance remains similar, Swin's performance increases substantially when we fine-tune all parameters. Intuitively, unfreezing the backbone allows 2D layers to adapt to cross-view fused features better. Therefore, we keep our backbone unfrozen in all experiments. %and Swin-B benefits more from this adaptation. Therefore, we keep our backbone unfrozen in all experiments.


%Specifically, freezing the ResNet-50 backbone shows similar mAP performance with a 0.6\% mIoU drop, while for Swin, freezing results in a 2.4\% mAP drop and 1.3\% mIoU drop. Intuitively, unfreezing the backbone allows 2D layers to adapt to cross-view fused features better and Swin-B benefits more from this adaptation. Therefore, we keep our backbone unfrozen in all experiments.

\noindent \textbf{Supplying 2D features directly to 3D models does not help:} Concatenating 2D features alongside XYZ+RGB as an input to Mask3D yields 53.8 mAP performance, comparable to 53.3\%\let\thefootnote\relax\footnotetext{$^{\dagger}$We do not use the expensive DB-SCAN post-processing of Mask3D, and hence baseline Mask3D gets 53.3 instead of 55.2 as reported by their paper} of the baseline model with only XYZ+RGB as input.

%We unproject 2D features from Resnet-50 and supply it as an additional input to Mask3D. We find that it results in a marginal increase in task performance. Thus, while always using 2D features might be a good idea, directly supplying these features to a 3D backbone might not be an optimal design as also shown by our 2nd ablation bullet. 

% \todo{Mention DBSCAN}

% \todo{1. no alternating. sharing weights and alternating 2d 3d, do we have this number?}
% \todo{2. no cross view fusion}
% \todo{joint 2d 3d}
% \todo{many 3d}
% \todo{2d backbone variation}
% \todo{no 2d pretraining}
% \todo{straightforward addition of 2d feats to mask3d}

% \subsection{zero shot??}





% \todo{make sure we bold numbers on tables}
% \begin{table}
% \caption{\textbf{Comparison on Scannet for Instance Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llccccc}

% Input & Model & mAP &  mAP50 & mAP25 \\ \hline
% \multirow{4}{*}{Sensor RGBD point cloud} & Mask3D $^{\dagger}$ & 43.9 & 60.0 & 69.9  \\
%  & Ours-Resnet50 & 45.7 & 66.3  & 81.8  \\
%  % & Ours-Swin-T &  &  &   \\
%  & Ours-Swin-L & 48.0 & 69.2 & 83.5  \\ \hline
% \multirow{2}{*}{Mesh Sampled point cloud} & SoftGroup & 46.0 & 67.6 & 78.9 \\
% & Mask3D & 55.2 & 73.7 & 83.5 \\
%  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table}
% \caption{\textbf{Comparison on Scannet for Semantic Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llc} 
% Input & Model & mIoU \\ \hline
% \multirow{8}{*}{Sensor RGBD point cloud} 
% & MVPNet & 68.3\\
% & BPNet & 69.7 \\
% & DeepViewAgg & 71.0 \\
%  & Ours-Resnet50 & 73.2  \\
%  % & Ours-Swin-T &    \\
%  & Ours-Swin-L & 76.0 \\ \hline
% \multirow{2}{*}{Rendered RGBD point cloud} & VMVF & 76.4 \\
% & Ours & \\ \hline
% \multirow{2}{*}{Mesh Sampled point cloud} & Point Transformer v2 & 75.4 \\
% & Swin3D-L & 76.7  \\
%  \hline
% \end{tabular}
% }
% \end{table}


% \begin{table*}
% \caption{\textbf{Comparison on Scannet200 for Instance Segmentation Task}}
% \label{tab:score-sim}
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{llcccccccccccc}

% Input & Model & \multicolumn{3}{c}{All} &  \multicolumn{3}{c}{Head} & \multicolumn{3}{c}{Common} & \multicolumn{3}{c}{Tail} \\
%  \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}  
% & & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25 & mAP &  mAP50 & mAP25\\ \midrule
% \multirow{3}{*}{Sensor RGBD point cloud} & Mask3D $^{\dagger}$ & 15.5 & 21.4 & 24.3 & 21.9 & 31.4 &  37.1 & 13.0 & 17.2 & 18.9 & 7.9 & 10.3 & 11.5 \\
%  & Ours-Resnet50 & 26.0 & 37.6 & 43.8 &  &  &  &  &  &  &  &  &  \\
%  % & Ours-Swin-T &  &  &   \\
%  & Ours-Swin-L (in progress) &     &         &   &  & & &   \\ \midrule
% \multirow{1}{*}{Mesh Sampled point cloud} & Mask3D & 27.4 & 37.0  & 42.3 \\
%  \midrule
% \end{tabular}
% }
% \end{table*}


% \begin{table}
% \caption{\textbf{Comparison on Scannet200 for Instance Segmentation Task}}

% \label{tab:score-sim}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{llccc}

% Input & Model  & mAP &  mAP50 & mAP25 \\ \midrule
% \multirow{3}{*}{Sensor RGBD point cloud} & Mask3D $^{\dagger}$ & 15.5 & 21.4 & 24.3  \\
%  & Ours-Resnet50 & 26.0 & 37.6 & 43.8  \\
%  & Ours-Swin-L &  30.0        &  43.0         &  51.0   \\ \midrule
% \multirow{1}{*}{Mesh Sampled point cloud} & Mask3D & 27.4 & 37.0  & 42.3 \\
%  \midrule
% \end{tabular}
% }
% \end{table}





% \todo{Maybe tables for other datasets, potentially from S3DIS/Matterport/Scannet200/Scannet++}

% \subsection{Joint 2D - 3D Training}



% \subsection{Downstream Application}





% \clearpage


% \section{Ablations}



% \todo{Let's not use the word panet, rather 3d fusion transformer}

% \adam{add qualitative results}

\subsection{Limitations}

Our experiments reveal the following limitations for \model{}: 

Firstly, like other top-performing 3D models, it experiences a notable performance drop when using sensor point cloud instead of the mesh point cloud. This issue arises from depth and camera pose noise, leading to misalignments between RGB-D and mesh data. In our future work, we aim to explore estimating depth and camera poses as part of the inference process, thus making our model more resilient to noise. 
Secondly, in this paper, we limited our scope to exploring the design of a unified architecture without scaling 3D learning by training on diverse 2D and 3D datasets jointly. We aim to extend this model to a unified 2D-3D open-vocabulary perception system that generalizes to in-the-wild scenarios akin to the current 2D perception systems.

%Our experiments reveal the following limitations for \model{}: First, \model{} (as well as other SOTA 3D models) have a sharp decrease in performance with sensor point cloud as input instead of the mesh point cloud. This is due to noise in depth and camera poses, resulting in misalignments between RGB-D and mesh. In our future work, we aim to explore inferring depth and camera poses as part of the inference process, thus making our model more resilient to noise. Second, the project's focus on investigating a unified architecture leveraging pre-trained features with both 2D and 3D data confines our experiments to small-scale datasets. Future efforts will involve scaling the model through training on diverse 2D and 3D datasets, incorporating free-flowing language and conducting comparisons with state-of-the-art open-vocabulary 3D models in a zero-shot setup.


%underperforms SOTA models . This is in part due to noise in depths, camera poses leading to misalignments between RGB-D and mesh. This limitation is also shared by other SOTA models, as demonstrated  by their sharp decrease in performance when using sensor poincloud as input. In our future work, we aim to explore inferring depth and camera poses as part of the inference process. 



% 1. Sensitivity to depth holes and noise
% 2. Sensitivity to pose errors. 
% These are shared by other point cloud models. 

% Our future directions will explore  inferring depth and camera poses as part of the 3d inference process. 

% this was just a first step to show that these kinds of architectures can work as well and even better than sota 3d specific model. another crucial next step is to scale up training jointly on more 2d and 3d datasets, and study open-vocabulary capabilities in 3d that the model can pick up from diverse datasets in 2D and compare against models that do post-hoc processing over 2d features like openscene. 


% we notice that perception significantly improves as we add more views, but maybe there are scenarios where we can't afford to have a ton of views. potentially generative models can utilize their priors to do completion in 3d and let us operate with less views



%A 3D perceoption model should
% \subsection{Maybe Experiments}:
% \begin{itemize}
%     \item Out of domain generalization
%     \item Training jointly on multiple 3D datasets
% \end{itemize}

==> 6_suppl_cvpr.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{Experiments}
\input{tables/test_real_in_domain_3d}
\subsection{Evaluations on ScanNet and ScanNet200 Hidden Test Sets} We submit \model{} to official test benchmarks of ScanNet \cite{scannet} and ScanNet200 \cite{scannet200}. Following prior works, we train \model{} on a combination of train and validation scenes. Unlike some approaches that employ additional tricks like DBSCAN \cite{mask3d}, ensembling models \cite{stratified}, additional specialized augmentations \cite{ptv2}, additional pre-training on other datasets \cite{swin3d}, finer grid sizes \cite{octformer} and multiple forward passes through points belonging to the same voxel, our method avoid any such bells and whistles.  

%We do not use any additional tricks, unlike other methods which employ additional and often not publicaly known bells and whistles like DBSCAN \cite{mask3d}, ensembling models \cite{stratified}, additional specialized augmentations \cite{ptv2}, additional pre-training on other datasets \cite{swin3d}, finer grid sizes \cite{octformer} and multiple forward passes through points belonging to the same voxel.  

The results are shown in \cref{tab:test_established_3d}. All conclusions from results on the validation set of these datasets as discussed in the main paper are applicable here. On the ScanNet benchmark, \model{} achieves close to SOTA performance on semantic segmentation and mAP25 metric of Instance Segmentation while being significantly worse on mAP metric due to misalignments between sensor and mesh sampled point clouds. On ScanNet200 benchmark, \model{} sets a new SOTA on semantic segmentation and mAP50/mAP25 metric of Instance Segmentation, while achieving close to SOTA performance on mAP metric. Notably \model{} is the first method that operates over sensor RGB-D data for instance segmentation and achieves competitive performance to models operating over mesh-sampled point clouds.

% \input{7_s3dis_m3d}

\subsection{ScanNet200 Detailed Results}
\input{tables/scannet200_detailed}

%ScanNet200 \cite{scannet200} splits the 200 object categories into three splits based on the frequency of their occurrence. These three splits are \textit{Head}, \textit{Common} and \textit{Tail} with 66, 68 and 66 categories respectively. We show a detailed breakup of ScanNet200 results presented earlier in \cref{tab:scannet200_ins} in \cref{tab:scannet200_detailed} on these splits.
ScanNet200 \cite{scannet200} categorizes its 200 object classes into three groups—\textit{Head}, \textit{Common}, and \textit{Tail}—each comprising 66, 68, and 66 categories, respectively. In \cref{tab:scannet200_detailed}, we provide a detailed breakdown of the ScanNet200 results across these splits. We observe that in comparison to SOTA Mask3D model trained on mesh-sampled point cloud, \model{} achieves lower performance on \textit{Head} classes, while significantly better performance on \textit{Common} and \textit{Tail} classes. This highlights the contribution of effectively utilizing 2D pre-trained features, particularly in detecting a long tail of class distribution where limited 3D data is available.
%We notice that \model{} underperforms the SOTA Mask3D model in \textit{Head} classes (especially on mAP metric), while much outperforming it on \textit{Common} and \textit{Tail} classes.   

\begin{figure}[t]
     \centering
     \includegraphics[width=0.48\textwidth]{figures/varying_views.pdf}
    \caption{ \textbf{2D mAP Performance Variation with increasing number of context views used}}
     \label{fig:num_views}
    % \vspace{-0.2in}
\end{figure}

\begin{figure*}[!ht]
     \centering
     \includegraphics[width=\textwidth]{figures/detailed_arch.pdf}
    \caption{ \textbf{Detailed \model{} Architecture Components}: On the \textbf{Left} is the 3D RelPos Attention module which takes as input the depth, camera parameters and feature maps from all views, lifts the features to 3D to get 3D tokens. Each 3D token serves as a query.  The K-Nearest Neighbors of each 3D token become the corresponding keys and values. The 3D tokens attend to their neighbours for L layers and update themselves. Finally, the 3D tokens are mapped back to the 2D feature map by simply reshaping the 3D feature cloud to 2D multi-view feature maps. On the \textbf{Middle} is the query refinement block where queries first attend to the text tokens, then to the visual tokens and finally undergo self-attention. The text features are optional and are only used in the open-vocabulary decoder setup. On the \textbf{Right} is the segmentation mask decoder head where the queries simply perform a dot-product with visual tokens to decode the segmentation heatmap, which can be thresholded to obtain the segmentation mask. In the Open-Vocabulary decoding setup, the queries also perform a dot-product with text tokens to decode a distribution over individual words. In a closed vocabulary decoding setup, queries simply pass through an MLP to predict a distribution over classes.}
     \label{fig:detailed_arch}
    % \vspace{-0.2in}
\end{figure*}





\subsection{Variation of Performance with Number of Views}
\label{subsec:num_views}
We examine the influence of the number of views on segmentation performance using the AI2THOR dataset, specifically focusing on the 2D mAP performance metric. The evaluation is conducted by varying the number of \textit{context} images surrounding a given \textit{query} RGB image. Starting from a single-view without any context (N=0), we increment N to 5, 10, 20, 40, 60, and finally consider all images in the scene as context. \model{} takes these $N + 1$ RGB-D images as input, predicts per-pixel instance segmentation for each image, and assesses the 2D mAP performance on the \textit{query} image. The results, depicted in \cref{fig:num_views}, show a continuous increase in 2D mAP with the growing number of views. This observation underscores the advantage of utilizing multiview RGB-D images over single-view RGB images whenever feasible.


\subsection{Inference Time}
We assess the inference time of Mask3D and \model{} by averaging the forward pass time of each model across the entire validation set, utilizing a 40 GB VRAM A100. When fed the mesh-sampled point cloud directly, Mask3D achieves an inference time of 228ms. When provided with the sensor point cloud as input, the inference time increases to 864 ms. This could be attributed to the additional computational overhead involved in transferring features from the sensor point cloud to the mesh-sampled point cloud before generating the output segmentation mask. Additionally, the sensor point cloud is typically larger than the mesh-sampled point cloud, as it also includes regions that were discarded during the mesh generation post-processing. \model{}-SwinB, which operates over the sensor point cloud, has an inference time of 960ms.

\section{Additional Implementation Details}


The detailed components of our architecture and their descriptions are presented in \cref{fig:detailed_arch}.  

More implementation details are presented below:

\noindent \textbf{Augmentations: } For RGB image augmentation, we implement the Large Scale Jittering Augmentation method from Mask2Former \cite{m2f}, resizing images to a scale between $0.1$ and $2.0$. We adjust intrinsics accordingly post-augmentation and apply color jittering to RGB images. Training involves a consecutive set of $N$ images, typically set to 25. With a 50\% probability, we randomly sample $k$ images from the range $[1, N]$ instead of using all $N$ images. Additionally, instead of consistently sampling $N$ consecutive images, we randomly skip $k$ images in between, where $k$ ranges from 1 to 4.

For 3D augmentations, we adopt the Mask3D \cite{mask3d} approach, applying random 3D rotation, scaling, and jitter noise to the unprojected XYZs. Elastic distortion and random flipping augmentations from Mask3D are omitted due to a slight drop in performance observed in our initial experiments.

\textbf{Image Resolutions}
We use a resolution of $240 \times 320$ for ScanNet, $480 \times 640$ for ScanNet200, and $512 \times 512$ for AI2Thor. In our AI2THOR experiments, we discovered that employing higher image resolutions enhances the detection of smaller objects, with no noticeable impact on the detection of larger ScanNet-like objects. This observation was confirmed in ScanNet, where we experimented with $480 \times 640$ image resolutions and did not observe any discernible benefit.

\textbf{Interpolation}
Throughout our model, interpolations are employed in various instances, such as when upsampling the feature map from $1/8$th resolution to $1/4$th. In cases involving depth, we unproject feature maps to 3D and perform trilinear interpolation, as opposed to directly applying bilinear interpolation on the 2D feature maps. For upsampling/downsampling the depth maps, we use the nearest interpolation. Trilinear interpolation proves crucial for obtaining accurate feature maps, particularly at 2D object boundaries like table and floor edges. This is because nearest depth interpolation may capture depth from either the table or the floor. Utilizing trilinear upsampling of feature maps ensures that if the upsampled depth is derived from the floor, it interpolates features from floor points rather than table points.

%Throughout our model, there are several places where we perform interpolations: for instance, while upsampling the feature map from $1/8$th resolution to $1/4$th. When we have depth, we unproject the feature maps to 3D and perform trilinear interpolation, instead of performing bilinear interpolation directly on the 2D feature maps. We use nearest upsampling to upsample the depth map to higher resolutions. Trilinear interpolation is important to get the correct feature map, especially at the 2D object boundaries like table and floor edge, since nearest depth upsampling can pick up depth from either the table or the floor. Doing trilinear upsampling of feature maps ensures that if the upsampled depth was picked up from the floor, it interpolates features from floor points and not the table points. 

\textbf{Use of Segments: }
Some datasets, such as ScanNet and ScanNet200, provide supervoxelization of the point cloud, commonly referred to as \textit{segments}. Rather than directly segmenting all input points, many 3D methods predict outputs over these segments. Specifically, Mask3D \cite{mask3d} featurizes the input points and then conducts mean pooling over the features of points belonging to a segment, resulting in one feature per segment. Following prior work, we also leverage segments in a similar manner. We observe that utilizing segments is crucial for achieving good mAP performance, while it has no discernible impact on mAP25 performance. We suspect that this phenomenon may arise from the annotation process of these datasets. Humans were tasked with labelling segments rather than individual points, ensuring that all points within a segment share the same label. Utilizing segments with our models guarantees that the entire segment is labelled with the same class. It's worth noting that in AI2THOR, our method and the baselines do not utilize these segments, as they are not available.

%Some datasets like ScanNet, ScanNet200 and Matterport3D provide supervoxelization of the point cloud, popularly known as \textit{segments}. Instead of directly segmenting all input points, most 3D methods predict outputs over these segments. Specifically, Mask3D featurizes the input points, and then performs mean pooling over the features of points belonging to a segment to get one feature per segment. We follow these prior works and also utilize the segments in the same fashion. We notice that using segments is important to get good mAP performance, while it does not affect mAP25 performance. 

\textbf{Post-hoc output transfer vs feature transfer: } \model{} takes the sensor point cloud as input and generates segmentation output on the benchmark-provided point cloud. In this process, we featurize the sensor point cloud and transfer these features from the sensor point cloud to the benchmark-provided point cloud. Subsequently, we predict segmentation outputs on this benchmark-provided feature cloud and supervise the model with the labels provided in the dataset. An alternative approach involves segmenting and supervising the sensor RGB-D point cloud and later transferring the segmentation output to the benchmark point cloud for evaluation. We experimented with both strategies and found them to yield similar results. However, as many datasets provide segmentation outputs only on the point cloud, transferring labels to RGB-D images for the latter strategy requires careful consideration. This is due to the sparser nature of the provided point cloud compared to the RGB-D sensor point cloud, and factors such as depth noise and misalignments can contribute to low-quality label transfer. Consequently, we opt for the former strategy in all our experiments.

\textbf{Depth Hole-Infilling: } The sensor-collected depth maps usually have holes around object boundaries and shiny/transparent surfaces. We perform simple OpenCV depth inpainting to fill these holes. We tried using neural-based depth completion methods and NERF depth-inpainting but did not observe significant benefits. 

\textbf{AI2THOR Data Collection: } AI2THOR \cite{ai2thor} is an embodied simulator where an agent can navigate within a house, execute actions, and capture RGB-D images of the scene. We load the structurally generated houses from ProcTHOR \cite{procthor} into the AI2THOR simulator, and place an agent randomly at a navigable point provided by the simulator. The agent performs a single random rotation around its initial location and captures an RGB-D frame. This process is repeated, with the agent spawning at another random location, until either all navigable points are exhausted or a maximum of $N = 120$ frames is collected. While ProcTHOR offers 10,000 scenes, we randomly select only 1,500 scenes to match the size of ScanNet. Additionally, we retain scenes with fewer than $100$ objects, as our model utilizes a maximum of $100$ object queries.


\begin{figure*}[!t]
\centering
    \includegraphics[width=0.95\textwidth]{figures/supp_qual_1.pdf}
    \caption{Qualitative Results on various 3D and 2D datasets}
    \label{fig:supp_qual}
    % \vspace{-0.3in}
\end{figure*}

% \begin{figure*}[!t]
% \centering
%     \includegraphics[width=\textwidth]{figures/supp_qual_2.pdf}
%     \caption{Qualitative Results on various 3D and 2D datasets}
%     \label{fig:supp_qual_small}
%     % \vspace{-0.3in}
% \end{figure*}

\section{Qualitative Results}
\cref{fig:supp_qual} shows qualitative visualizations of \model{} for various 3D and 2D datasets.

==> 9_contribution.tex <==
\section{Contribution Statements}
\textbf{Ayush Jain} conceived the idea and led the project. He was responsible for the majority of the code development, design of the interleaving 2D-3D layers in the architecture, setting up datasets and baselines and writing sections of the paper.  

\noindent \textbf{Pushkal Katara} helped with initial experiments, baselines, codebase and paper figures

\noindent \textbf{Nikolaos Gkanatsios} played a pivotal role in the initial brainstorming of this direction, formalized the 3D RelPos Attention Transformer, wrote sections of the paper and continually contributed to research discussions.

\noindent \textbf{Adam W. Harley} led weekly advisory meetings, played a key role in identifying crucial conceptual bugs (e.g., emphasizing voxelization for consistent neighborhood structure across the varying number of views, identifying critical issues in early attempts with bird's-eye view cross-attention), and advised on low-level implementation details. He also significantly contributed to re-writing the initial draft of the paper.

\noindent \textbf{Gabriel Sarch} conceptualized and led the embodied instruction following experiments. 

%\noindent \textbf{Kriti Aggarwal} met bi-weekly for research discussions, led the collaboration with the Microsoft Turing team and played a key role in helping with GPU resources from the Microsoft Team. 

\noindent \textbf{Kriti Aggarwal} and \textbf{Vishrav Chaudhary} led the collaboration with the Microsoft Turing team and provided early feedback on the project direction.

\noindent \textbf{Katerina Fragkiadaki} advised and directed the project development, proposed the pivotal idea of unifying 2D-3D perception with RGB-D as a 3D representation, contributed to brainstorming and asking the hard questions that led to research insights, secured project funding, and authored sections of the paper.

==> OLD0_abstract.tex <==
\begin{abstract}


Contemporary 3D perception datasets, such as ScanNet, Matterport, and S3DIS, benchmark segmentation and labeling of  3D colored meshes from  indoor scenes, obtained through post processing of sensed multiview RGB-D images. % to estimate camera poses and  3D meshes. 
The state-of-the-art  in these benchmarks belongs to models that consume the dataset-provided 3D point clouds directly, instead of the sensed RGB-D images that generated them. % and forego any image-centric featurization;    
They typically %do not use any 2D pre-training, 
%rather they are trained within each dataset and in fact 
%and they  
outperform alternatives that featurize the posed RGB-D multiview  images instead.  
This gap in performance %between methods that consume images and 3D point clouds   
has 
fueled the belief that 2D and 3D visual understanding  should be addressed with distinct model architectures. In this paper we challenge this view and %instead explore the unification of 2d and 3d perception 
%attempt to explain this paradox of 3D vision datasets being dominated by within domain %models as opposed to benefitting from foundational feature image pre-training. 
 propose \model{}, a  model that can segment and label both  2D RGB images  and  3D point clouds.%, using  posed RGB-D image collections. %, to segment and label both images and corresponding 3D point clouds.  
 \model{} takes as input alternates between fusing information within views and fusing information across views. % image view 
 %with 2D convolutions or 2D relative attentions,  
% and across views.% and eventually segments the image or 3D feature clouds. 
 It differentiates single-view and multi-view input only through positional encodings, which capture pixel coordinates of 2D patch tokens % during within-image fusion 
 and  3D coordinates of 3D feature tokens. % during cross-view fusion.  % with 3D relative attentions. 
 \model{} achieves state-of-the-art performance on  ScanNet200 and Alfred 3D object instance benchmarks, and competitive performance on ScanNet,  Matterport, and  COCO. With extensive ablations, we quantify the contribution of pre-training the 2D image backbone, alternating 2D and 3D feature fusion, and training jointly across 2D and 3D data. %and   in \model{}. %We show cross-view fusion is important for 3D instance segmentation but less for 3D semantic segmentation. 
 Our model outperforms all previous works by a wide margin when the sensed 3D point cloud is used in place of the dataset-provided mesh vertices. %, and thus there is no noise during the unpro which suggests that %, which explains the good performance of methods that distill per view 2D foundational features  into 3D differentiable feature fields.  
 When used as the 3D perception engine  in an instructable embodied agent architecture, it sets a new state-of-the-art on the TEACH action-from-dialogue benchmark. % In simulated environments our model much outperforms point cloud models and sets a new state of the art in the TEACH benchmark when used as the perception backbone of an embodied instruction following agent. 
 %Our model experiments shed light to the paradox of processing provided meshes versus RGB-D image views  suggesting that misalignment between posed image views and 3d meshes may be to blame for lower performance, suggesting new ways of evaluating 3D perception.
%We believe our model makes a step towards unifying 2d and 3d perception models





%Current state-of-the-art (SOTA) 3D computer vision methods rely on domain-specific architectures and small-scale datasets, leading to limited generalization. In contrast, 2D models trained on diverse data perform well in real-world scenarios. Motivated by this, we propose a single unified vision model using 2D techniques. Our model offers improved generalization, performance, and versatility by training on both 2D and 3D datasets. Experimental results on the Scannet benchmark demonstrate superior performance compared to domain-specific architectures. Secondly, it exhibits enhanced generalization capabilities by successfully adapting to new 3D scenes outside the training domain, surpassing the limitations of existing Scannet-based models. Lastly, the model showcases the ability to jointly train on both 2D and 3D datasets, achieving SOTA results in both domains. These findings highlight the potential pathway of building unified vision foundation models by excelling in multiple domains and enabling seamless integration of 2D and 3D data.
\end{abstract}


==> OLD1_introduction.tex <==
\vspace{-0.1in}
\section{Introduction}
%\vspace{-0.1in}
%\topic{the paradox of 2d pretraining not helping and the sota being small within domain pointcloud models}
% \todo{AYUSH: add all citations in the intro, add footnote on the odin name, give fedback.}

There has been a lot of recent excitement and research interest in porting 2D foundational image features to 3D scene understanding \cite{conceptfusion,openscene,openmask3d,semabs,vlfield,pla,lerf,pl,deepview}. \adam{having a pile of citations in a row is bad}
%\todo{lets list all different categories of methods that attempt this}
Some methods  lift  pre-trained 2D image features using sensed depth into 3D feature clouds or voxelised 3D feature maps \cite{openscene,openmask3d,deepview,pla}, and others distil 2D feature backbones to  differentiable parametric 3D models,  such as NeRFs,  by training  them per scene to ``render" 2D  image feature maps of pretrained 2D backbones \cite{lerf,pl}.  These efforts are supported by the continual improvement of pre-trained 2D image features through large-scale weakly supervised image captioning  \cite{clip,captiongenerator} or  image generation \cite{dalle,MAE}. \ayush{None of them use DALL-E or MAE features. most of them use clip or openseg/lseg which is clip fine-tuned on coco. should i still cite the ones you mention? what is captiongenerator?} Empirical evidence shows that large-scale 2D pre-training is instrumental for performance in several 2D downstream tasks, such as 2D image segmentation and labelling \cite{}. \ayush{i am thinking of SAM, Mask2Former: they don't do pre-training but rather train themselves on large data; which 3d would never have. do you have some paper in mind to cite? (i have some ego-centric papers in mind that use MAE for sota). infact kaiming he's paper: https://arxiv.org/abs/1811.08883 says pre-training in 2D only helps in convergence speed and not accuracy. I think we should motivate by saying: 2D has lots of data, 3D doesn't, can we take advantage of 2d data? one straightforward way is to use 2D features, other is joint training with 2D} Paradoxically, and in stark contrast to the 2D domain,  
%Despite these efforts and the , 
the state-of-the-art %in 3D instance segmentation and labelling %object detection and pixel labelling 
in established 3D segmentation benchmarks such as ScanNet \cite{scannet} and ScanNet200 \cite{scannet200} are  models that operate directly on the dataset-provided 3D point clouds and trained in-domain, without any image featurization and related pre-training \cite{mask3d,maft}. %\todo{do we want to give an example of performamce between lets say openfusion and } %For instance, zero-shot 2D foundational model for 3D only address 3D semnaitc  labelling and obtain such and such score, while an in-domain train Mask3d model attains . 


We see several benefits in foregoing dataset-provided 3D meshes and instead operate directly from the posed RGB-D images. First, %3D mesh 
%that geenrated them:  instead. preprocessing:  processing steps arequite involving and 
in several real-world applications we need agents to function directly from incomplete posed RGB-D input, bypassing involving and time consuming post-processing. Second, it would let us use large pre-trained (foundational) 2D  image backbones for 3D perception. Third, it would bring the research communities of 2D and 3D perception  closer, allowing models to transfer across the two. Yet, getting good results  from raw posed RGB-D data hasn't worked well in these benchmarks  due to misalignments and noise between camera poses and the labelled 3D meshes \cite{virtualview,deepview}. %  thus undermining this direction, and  % together by using RGBD and thus could pursue a single architecture. 
This performance gap has nourished the idea that 2D and 3D perception are indeed very different in nature and should be addressed with distinct neural models. %, justified by the fact that images and 3D point clouds are very different in nature.   
% \ayush{maybe we should say somewhere here or later that we benchmark prior methods and our methods with sensor PC as input too?}
%It has been argued that  building foundational models of 3d perception  would   require a very large 3D (complete multiview data) annotated data, currently unavailable \cite{}.
%Indeed, 3D perception research has evolved often independently from 2d image one, proposing architectures that consume 3D point cloud data, such as PointNet, Minkowsi convolutions, Swin 3d or 3d point transformers that are types of graph neural networks on 3D point graphs. 
Indeed, it is unimaginable that a model can be shared across both 2D and 3D visual understanding.
%given that images and 3D point clouds are very different in nature, and so far models have been developed to consume one or the other type of input. 
Recently, Omnivore \cite{omnivore} introduced a unified visual model for images, videos, and single-view 3D. However, it focuses solely on classification tasks and does not extend to the more challenging tasks of semantic and instance segmentation. %\cite{butd} proposed an architecture that works on both 2D and 3D domains for the referential grounding task. However, they train their model independently in 2D and 3D, partly because the input representation of pointclouds in 3D and RGB images in 2D, do not allow the use of a unified visual backbone


%\todo{Notable exception is omnivore \cite{} but it only addresses the image labelling task, not instance  segmentation and labelling. +++} 


%\todo{\model{} can also stand for Omni Dimensional Instance Segmentation if we want to use it}

In this paper, we challenge this view and propose \model{}$^{\dagger}$\let\thefootnote\relax\footnotetext{$^{\dagger}$ Inspired by Norse God Odin's sacrifice of his eye for wisdom, we name our model Odin as it sacrifices mesh input to unify 2D and 3D.}, a model for 2D and 3D object segmentation and labelling that can consume both 2D single images and multiview posed RGB-D ones, with SOTA or close to SOTA performance across both 2D and 3D object instance segmentation in multiple benchmarks.   
%ask the question: Is 2D and 3D perception indeed that different? After all, a 3D scene pointcloud is simply an accumulation of depth-augmented images from multiple viewpoints, and it is not god-given or benchmark-provided as it appears in today's 3d perception benchmarks. 
\ayush{maybe its a bad idea to stress that we are relative position transformer?: our panet layers are relative but not the rest.}
 \model{} is a relative position transformer that  alternates between 2D within-image fusion using 2D convolutions or 2D attentions and 3D cross-view fusion using 3D attentions. 
 %is a relative position transformer 
 %that
 The main difference between 2D and 3D fusion operations is the 
 %can consume both 2D RGB images and a variable number of posed RGB-D images with the sole difference being
 the positional encoding of the tokens involved: in 2D image fusion, the feature positional encoding reflects $(x,y)$ pixel coordinates of the 2D tokens, while in cross-view fusion the positional encoding reflects $(X,Y,Z)$ 3D scene coordinates of the 3D tokens. We use relative position attention operations in  3D to gain  invariance to the center of the coordinate system. We use $K$-NN neighborhoods in 3D attentions to avoid the quadratic cost of all-to-all attention in 3D. \model{} greatly benefits from  2D feature pre-training of its 2D fusion weights, as well as co-training across both 2D and 3D data. %is pre-trained in a weakly-supervised fashion.  %Our 2D feature backbone is a large  pre-trained and then lifted for the 3D cross view transformer. 

We test \model{} for 2D/3D instance segmentation and 3D semantic segmentation, covering the 2D COCO object segmentation benchmark, and the 3D benchmarks of ScanNet \cite{scannet}, ScanNet200 \cite{scannet200}, and Ai2Thor \cite{ai2thor,procthor}. \model{} achieves state-of-the-art performance in ScanNet200 and Ai2Thor 3D benchmarks and obtains close to SOTA performance in ScanNet and COCO benchmarks. Notably, it outperforms all prior methods in all 3D benchmarks when tested using sensor RGB-D point cloud as input. We show our model's ability to train jointly on 3D and 2D datasets, which results in performance increase in 3D benchmarks while maintaining close to SOTA performance in COCO benchmark. This results in a unified model that, at test time, can work on both single-view 2D and multiview RGB-D input, thus bringing the 2D and 3D modalities closer together.


%We test \model{} for 2D/3D instance segmentation and 3D semantic segmentation  and in the 2D COCO  object segmentation benchmark and in the 3D benchmarks of ScanNet \cite{scannet}, ScanNet200 \cite{scannet200} and Ai2Thor \cite{ai2thor,procthor}.  \model{} achieves state-of-the-art performance in ScanNet200 and Ai2Thor 3D benchmarks, and close to SOTA performance in ScanNet and COCO benchmarks. It outperforms all prior methods in all benchmarks when all methods are tested using sensor RGBD pointcloud as input. We show our model's ability to train jointly on 3D and 2D datasets, which results in performance increase in 3D benchmarks while maintaining close to SOTA performance in COCO benchmark.

%\model{} achieves SOTA performance in ScanNet200 and close to SOTA in ..., while maintaining SOTA 2D COCO mAP. 

Our ablations show that co-training across both 2D and 3D examples helps boost 3D performance, and the model improves with the capacity of the pre-trained backbone. We empirically show that alternating across 2D and 3D fusion outperforms more straightforward architectures of first fusing in 2D and then in 3D. % feature fusion, without alteration between the two. 

\todo{what about adding 2d features to ask3d?} \ayush{it marginally helps them, we can skip this from intro i think, but don't have any strong opinions} Directly feeding 2D features to SOTA Mask3D \cite{mask3d} achieves similar performance as the variant without 3D features.

Our comparisons against 3D point cloud methods \cite{mask3d} suggest that  performance of the latter varies significantly with the quality of the 3D input point cloud;  \model{} greatly outperforms point cloud  models  when all models use the sensed 3D point cloud assembled from posed RGB-D images directly, in place of the dataset-provided 3D mesh.  
Our comparisons  against methods that lift and average 2D foundational features across views show that though this suffices for 3D semantic segmentation, cross-view fusion is essential for 3D instance segmentation, where \model{} shines over all alternatives. 
\ayush{i added openscene comparisons, and also we have virtual view etc, but their results are only on semantic and not instance segmentation -- so we cannot say anything about instance segmentation from those exps. The only exp which supports the above line is an ablation we do -- and we can just say that while this strategy is very popular, we find that it is suboptimal for instance segmentation through our ablations}
% that does not suffer from misalignments between estimated poses and 3D mesh, our model outperforms 3D point cloud methods and sets a new state-of-the-art in the TEACH instruction following benchmark 
When used as the 3D object segmentor of a SOTA embodied 
agent model \cite{helper} in the simulation ALFRED \cite{alfred} and TEACh benchmark \cite{teach} in the setup with access to RGB-D and pose information from the simulator,  our model sets a new state-of-the-art in the Alfred and TEACh instruction-following simulation  benchmark. We finally  show the sensitivity of our model and 3D baseline models to depth noise and poses errors, and present directions for future work.  \ayush{i think we don't really say anything deep about noise and pose through our exps apart from the fact that all models suffer from it. also the temporal order of this line should be much earlier -- because the sense depth exp is the first thing we show}
We will make our models and code publicly available upon publication. 



% used
%suggest several key conclusions:  
%1) The performance of 3D poincloud models, such as Mask3D, varies a lot depnding on whether they are trained and tested on the 3D mesh provided by the benchmark, the 3D point cloud assembled from rendered 3D deth maps, or the pointcloud assembled from sensed RGB-D images, with a continuous degradation in performance. Our model is close to mask3d in given mesh and much outperforms it in the rendered and sensed depth case across datasets.
%2) In simulation environments, where depth does not suffer from noise, our model outperforms 3D point cloud models across the board, suggesting that slight misalignments between 3d mesh and sensed RGB-D views may be to blame for performance. We set a new state of the art in \cite{} simply by replacing the per view detector and tracker of the leading method with our 3d perception system
%3) Our 3d performance improved when the model is cotrained with 2D data, showing a synergy not only through pretrained features but also through data concatenation
%4) Our model improves with higher capacity of the 2D pretrained backbone.


%When mask3d is trained and tested not in the dataset provided mesh 
%First, we show that our model is close to SOTA mask3d 

%We argue what differs between 2d and 3d data is the  additional depth channel that can be , essentially changing the 


%But we argue that 3d and 2d are close. 3d meshes came from images, they are not god given. So, we seek a modle that can consume a variable number of input views and their depth prediction.  how can 2d feature pertaining  

%segmentation as a unified task between 2D and 3D instead of bounding boxes


%In recent years, significant advancements in the field of computer vision have been driven by the scaling up of models and the utilization of vast amounts of data. However, when it comes to 3D data, the challenges of collection and annotation have hindered the progress of scaling up 3D model learning. Unlike their 2D counterparts, 3D models often struggle to generalize effectively across domains. This limitation raises the question of how we can bring 3D and 2D models closer together to enable the direct sharing of data and parameters, given the abundance of labeled 2D data and the availability of robust architectures.

%One popular perspective within the research community suggests moving away from scaling 3D models and instead exploring the use of 2D foundation models to tackle 3D perception. These models focus on freezing the weights learned from 2D data and subsequently employing them per view, with simple fusion techniques applied. While they show impressive results in zero-shot settings, they significantly underperform compared to domain-specific 3D architectures when tasked with processing 3D information. Consequently, it becomes crucial to investigate how multiview methods can be developed to bridge the performance gap and enable the sharing of 2D-3D data and architectures.

%While previous attempts have been made to employ 2D-based multiview methods on datasets such as ScanNet, their conclusions have shown that these methods are generally inferior to dedicated 3D models. \cite{} showed that when using rendered views, larger camera field of view and active view sampling, the performance of these methods can approach that of domain-specific models. Notably, most of these approaches have focused on semantic segmentation, where the objective is pixel-wise labeling, rather than instance labelling, which requires substantial cross view reasoning to associate same instance of an object across multiple views. In fact, the only RGB-based method available on Instance Segmentation Benchmark of Scannet is MaskRCNN, which was introduced back in 2017. Therefore, in order to develop comprehensive architectures that can effectively share 2D-3D data and architectures, it is essential to study the development of multiview methods capable of achieving comparable performance to 2D models.


%In this work, we aim to take a significant step towards addressing this challenge by proposing a novel multiview RGBD model. Our model achieves close-to-state-of-the-art results on the ScanNet benchmark for both semantic and instance segmentation. Moreover, we demonstrate that our model exhibits better generalization capabilities compared to domain-specific models when dealing with out-of-distribution scenes. Furthermore, our model can be stably trained on both 2D and 3D data, enabling it to process various inputs during testing, including single RGB images, video sequences, and image sequences with depth information. While our approach does not achieve the current state-of-the-art performance, our findings suggest that a multiview RGBD approach holds promise as a viable solution for enhancing 3D perception. Consequently, this approach has the potential to scale 3D perception across diverse classes and facilitate real-world applications.


==> OLDmethod.tex <==
\begin{figure*}[!ht]
     \centering
     \includegraphics[width=\textwidth]{figures/method.png}
    \caption{ \textbf{\model{} Architecture}}
     \label{fig:method}
    % \vspace{-0.2in}
\end{figure*}
\todo{we need a figure that somehow very easily shows alternation between 2d fusion and cross view 3d fusion, this architecture doesnt show that. i find it very hard to uderstand what si going on here, maybe we share some diagram on paper first before making keynotes?}

\adam{figures 1-2 are hard to read (export pdf instead of png) and have too much whitespace. packing things tighter will also make the text relatively larger, which is important too.}

\section{\model{}}
\model{}'s architecture is shown in \Figure-\ref{fig:method}. It can take as input a single 2D RGB image or a posed RGB-D image sequence (images associated with depth maps and known camera parameters) and output the corresponding 2D or 3D instance segmentation masks and their semantic labels --- per 2D pixel or 3D point respectively. To achieve that, \model{} extracts multiscale features for each input image separately and then alternates between a 2D convolution-based or attention-based within-view fusion (shown in BLA color in Figure \ref{fig:method}) and a 3D attention-based cross-view fusion (shown in BLA color in Figure \ref{fig:method}). A segmentation decoding head predict instance masks and semantic labels from the final fused features. Notably, \model{} shares the majority of its parameters across both RGB and multiview RGB-D inputs. We detail the components of our architecture below.

%Our model can handle both 2D and 3D inputs, predicting per-pixel segmentation masks for the input pixels.  In the case of a 2D input, the model receives a single RGB image, while for a 3D input, a sequence of multiview RGB images, depth maps, and camera parameters serve as input.  The input undergoes processing through a UNet\cite{unet}-like backbone, yielding features across multiple scales. Subsequently, we instantiate distinct \textit{instance queries}, each tasked with predicting the segmentation mask and class label for an individual object instance within the scene. Notably, the majority of the architecture shares common parameters for both 2D and 3D inputs. 

%\todo{THIS IS THE WRONG WAY TO PRESENT IT, SAY: WE TAKE AS INOPTU THIS, WE PROCESSING IT IN 2D LAYER, THEN WE ALTERNATIVE BEWEEN 3D AND 2D FUSION,. OUR 2D FUSION IS CNVOLUTIONS OR BLA, OUR 3D FUSION IS 3D RELATINE KNN ATTENTIONS. NEXT WE DESCRIBE DETAILS. NO NEED TO MENTION QUERIES IN THE ZOOM OUT PARA.} 


%However, for multiview 3D input, we introduce additional layers to facilitate the fusion of features across views. Furthermore, 2D positional encodings are utilized during attentions when processing 2D inputs, whereas 3D positional encodings are applied when handling 3D inputs. We describe each of the components in our architecture below.

%Figure-\ref{} illustrates the architecture of \model{}. Our model can handle both 2D and 3D inputs, predicting per-pixel segmentation masks for the input pixels.  When the input is 2D, our model takes a single RGB image as input. When the input is 3D, our model takes as input a sequence of multiview RGB images, depth maps, and camera parameters. We pass the input through a UNet\cite{unet}-like backbone to obtain features at multiple scales. Then, we instantiate some \textit{instance queries}, each being responsible for predicting the segmentation mask and class label for a single instance of an object in the scene. For both 2D and 3D inputs, the majority of the architecture shares all parameters. For 3D input, we add some additional layers which fuse features across views. We also use different positional encodings in 2D and 3D. 

%\subsection{Backbone with Cross-View Contextualization} 

\textbf{Within-view fusion with 2D backbones} We use a pre-trained 2D backbone like ResNet \cite{resnet}  or Swin Transformer \cite{swin}, following Mask2Former \cite{m2f}, a state-of-the-art 2D segmentation model. When only a single RGB image is available, we directly pass it through the backbone to obtain features at multiple scales.

\textbf{Cross-view fusion with 3D relative K-NN Transformer} When a posed RGB-D sequence is available, we interleave the 2D backbone's blocks with \textit{Point Attention Layers} to perform early cross-view contextualization of features, as shown in Figure-\ref{fig:method}. The goal of this fusion is to make the individual images' representations consistent across views and more robust to factors like surrounding context, lighting variations and occlusions. As we show in our experiments, feature consistency of a 3D object across views is essential for helping the instance segmentation head to easily classify the whole object as one instance, instead of over-segmenting the object into multiple instances.

Point Attention is a local \textit{neighbourhood-attention} layer, similar to Point Transformers \cite{ptv1, ptv2}. Specifically, we first unproject the multiview 2D features to 3D using the depth and known camera parameters and voxelize the unprojected feature point cloud. 
Then, each voxel point attends to its $K$ nearest neighbors. The positional embeddings for the keys and values in this attention are relative to the query point's location, by simply encoding the distance vector between a point and its neighbour with an MLP, thus making a Point Attention layer invariant to translation. While each point always attends to the same $K$ neighbors, its effective receptive field keeps growing since the neighbors also update themselves by attending to their neighbors. 
Finally, we de-voxelize the feature cloud and rearrange the features back into multiview 2D feature maps for further 2D processing. We show a detailed architecture of a Point Attention layer in Figure-\ref{fig:method}.

%\subsection{BackBone with Cross-View Contextualization} We closely follow Mask2Former \cite{m2f} in designing our backbone. We start with a pre-trained image-based backbone like ResNet \cite{resnet} or Swin \cite{swin}. In the 2D case, we just pass the input image through this image-based backbone to obtain features. In the 3D case, we have RGB images from multiple views in the scene. We can simply batch these images and pass them through the image-based backbone to obtain per-view features. However, these features are not 3D consistent since each image is featurized independently of other images. This implies that the same instance of a 3D chair, seen from multiple views, can have very different features based on the unique context, lighting conditions and occlusions of these individual images. As we show in our experiments, feature consistency of a 3D object across views is essential for helping the instance segmentation head to easily classify the whole object as one instance, instead of over-segmenting the object into multiple instances. Moreover, this design does not utilize multiview information effectively -- an object might be clearly visible in one view while very heavily occluded in the other view. Hence, to perform early cross-view contextualization of features, we utilize \textit{Point Attention Layers}.

%\textbf{Point Attention Layers (PANets):}
%\textbf{Cross-view fusion with 3D relative K-NN Transformer}
%In the 3D scenario, we have access to multiple RGB views of a scene. A straightforward batch processing of these images through the image-based backbone does not guarantee 3D consistency in the extracted features. Specifically, features for a given 3D object, like a chair, may differ significantly across views influenced by various factors like surrounding context, lighting variations and occlusions. Moreover, fusing features from multiple views can help exploit the benefits of seeing an object from multiple views. Hence, we utilize \textit{Point Attention Layers} to perform early cross-view contextualization of features.
%\todo{START WITH THE LAST SENTENCE: JUST FIRST SAY WHAT YOU DO, AND THEN JUSTIFY WHY THIS HELPS.} 
%These layers take features from distinct views of a scene as input and output multiview-consistent features by contextualizing the features from all views with each other. This operation is similar to self-attention, however, a naive attention to all points can quickly become very expensive in typical 3D scenes with large number of points. Hence, we employ a local \textit{neighbourhood-attention} similar to Point-Transformers \cite{ptv1, ptv2}. Specifically, we unproject the multiview 2D features to 3D by using the depth and camera parameters and voxelize the unprojected feature pointcloud. For each voxel point, we identify its $K$ nearest neighbors and execute vanilla multihead cross-attention from the voxel point to its K-nearest neighbors. Positional embeddings for the keys and values in this attention are relative to the query point, by simply encoding the distance vector between a point and its neighbour with an MLP. While each point always attends to the same $K$ neighbors, its effective receptive field keeps growing since the neighbors also update themselves by attending to their neighbors. Finally, we de-voxelize the feature cloud and rearrange the features back into multiview 2D feature maps for further 2D processing. We show a detailed architecture of PANet Layers in Figure-\ref{fig:method}.

%\textbf{Point Attention Layers (PANet)}: The input to these layers are features from individual images -- potentially featurized independent of other images and the goal is to produce multiview consistent features. Naive attention to all points can quickly become very expensive in typical 3D scenes. Hence, we employ a local \textit{neighbourhood-attention} similar to Point-Transformers \cite{ptv1, ptv2}. Specifically, we unproject all features to 3D by using the depth and camera parameters and voxelize the unprojected pointcloud. For each voxel point, we find its $K$ nearest neighbours and do vanilla multihead cross-attention from the voxel point to its K-nearest neighbours. For positional embeddings in this attention, we encode the relative distance vector between the center point and the neighbour by an MLP. We perform multiple layers of this K-NN attention, and while the neighbors of a specific point remain fixed throughout these multiple layers, the effective receptive field keeps expanding through the feature updates of the neighbors from their neighbours. \\
%\textbf{Alternating 2D and 3D fusion}
Interleaving within-view and cross-view fusion layers, we can utilize the pre-trained features from the 2D backbones while also fusing features across views to make them 3D consistent. 


\textbf{Upsampling} The 2D backbone interleaved with Point Attention layers gives us feature maps of multiple scales (resolutions). Following Mask2Former\cite{m2f}, we perform multiscale within-view deformable attention among the three lowest-resolution feature map scales $(1/32, 1/16, 1/8)$. When the input is multiview RGB-D and thus 3D information is available, we apply an additional Point Attention layer at each scale to restore cross-view consistency after within-view deformable attention.
Finally, we use a simple upsampling layer on the $1/8$th resolution feature map with a skip connection from the backbone to obtain the final feature map at $1/4$th resolution. While bilinear interpolation suffices when upsampling 2D feature maps, we find trilinear interpolation to perform empirically in the multiview case.

For several 3D benchmarks like Scannet \cite{scannet}, the objective is to label a point cloud derived from a mesh rather than the sensor point cloud. Consequently, on those benchmarks, instead of upsampling the $1/8$th resolution feature map to $1/4$th, we trilinearly interpolate features from $1/8$th resolution feature map to the provided point cloud. Additionally, we trilinearly interpolate the features from $1/4$th resolution feature map in the backbone to the point cloud and use it as a skip connection. 

%\todo{maybe describe ghost transfer here -- for that we would need to explain that setup before, which is ok}

\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.3]{figures/components.png}
    \caption{\small\textbf{Components} of \model{}}
    \label{fig:model_components}
\end{figure}

%\paragraph{Transformer Decoder}
\textbf{Segmentation head} Our segmentation head builds upon Mask2Former \cite{m2f} and is shared between 2D and 3D, with the exception of the positional embeddings. It is a Transformer decoder architecture that takes as input the upsampled feature maps and outputs segmentation masks and classes for the instances in the scene. We instantiate a set of $N$ learnable object queries as slot vectors, responsible for decoding individual instances. These queries are iteratively refined by a \textit{Query Refinement} block which consists of cross-attention to the upsampled features, followed by a self-attention layer among the queries. To distinguish between the 2D (input is an image) and the 3D (input a posed RGB-D sequence) case and sufficiently exploit the available information, we use different types of positional encodings in the cross-attention layer. Specifically, we use Fourier positional encodings in 2D, while in 3D, we encode with an MLP the XYZ coordinates of the unprojected feature cloud of the corresponding resolution. The refined queries are used to predict instance masks and semantic classes. For mask prediction, the queries do a pixel-wise or point-wise dot-product with the highest-resolution upsampled feature map or cloud respectively. For semantic class prediction, we use an MLP over the queries, mapping them to class logits.

%These queries cross-attend to a feature map from the upsampler, self-attend with each other and then do dot-product with the highest resolution feature map scale to produce a per-pixel segmentation mask. Following Mask2Former, in each layer, the queries cross-attend to one of the three coarsest feature map resolutions $(1/32, 1/16, 1/8)$ starting from lowest resolution to higher resolution, followed by self-attention and then dot-product with feature map at $1/4$th resolution. For cross-attention from queries to features, we use the masked-attention strategy from Mask2Former which attends only within the foreground region of the predicted mask for each query. In cross-attentions, we use fourier positional embeddings for the features in the 2D case. With 3D input, we use learnable positional encoding where we encode the unprojected $N X 3$ points using an MLP. Thus, the entire transformer decoder is shared across 2D and 3D, except for the positional embeddings. 

\textbf{Open vocabulary mask decoding:} We additionally propose an alternative segmentation head to enhance flexibility to an arbitrary number of semantic classes and accommodate for training on multiple datasets jointly, inspired by previous works on open-vocabulary detection \cite{butd,glip,xdecoder}. 
We supply the model with a \textit{detection prompt} formed by concatenating object categories into a sentence (e.g., \textit{``Chair. Table. Sofa."}) and encode it using RoBERTa \cite{roberta}. In the query-refinement block, queries additionally attend to these text tokens before attending to the upsampled feature maps. For semantic class prediction, we first perform a dot-product operation between queries and language tokens, generating one logit per token in the detection prompt. The logits corresponding to prompt tokens for a specific object class are then averaged to derive per-class logits. This can handle multi-word noun phrases such as \textit{``shower curtain"}, where we average the logits corresponding to \textit{``shower"} and \textit{``curtain"}. The segmentation masks are predicted by a pixel-/point-wise dot-product, in the same fashion as described earlier.

% \textbf{Open vocabulary mask decoding:} For instance class prediction, Mask2Former utilizes an MLP over the queries, mapping them to the dimension of the number of classes, and supervised by a softmax loss. However, this approach confines the model to a fixed vocabulary, posing challenges when training jointly on datasets with distinct category labels. To enhance flexibility and accommodate training on multiple datasets jointly, our model design aligns with BUTD-DETR \cite{butd}, GLIP \cite{glip}, and X-Decoder \cite{xdecoder}. We supply the model with a \textit{detection prompt} formed by concatenating object categories into a sentence (e.g., Chair. Table. Sofa.) and encode it using RoBERTa \cite{roberta}. In the query-refinement block, queries attend to these text tokens before doing the usual cross-attention to visual tokens and self-attention. For predicting the segmentation mask, these queries do a pixel-wise dot-product with the highest resolution feature map from the upsampler (1/4th resolution or the features transferred to provided point cloud). For class prediction, the queries perform dot-product with the language tokens, generating one logit per sentence token. The logits corresponding to sentence tokens for a specific object class are then averaged to derive per-class logits, supervised by the vanilla cross-entropy loss (for e.g. by averaging the logits of ``shower" and ``curtain" to obtain the logit for the ``shower curtain" class). 

\textbf{Training details} 
We initialize our model with pre-trained weights from Mask2Former \cite{m2f} trained on COCO \cite{coco}. Subsequently, we train all parameters, encompassing both pre-trained and new parameters from cross-view layers. During training in 3D scenes, our model processes a sequence of $N$ consecutive frames, usually comprising 25 frames. At test time, we input all images in the scene to our model, with an average of 90 images per scene in ScanNet. During training, we employ open vocabulary mask decoding for joint 2D and 3D datasets and vanilla closed-vocabulary decoding otherwise. Training continues until convergence on 2 NVIDIA A100s with 40 GB VRAM or 2 NVIDIA A6000s with 48 GB VRAM, with an effective batch size of 6 in 3D and 16 in 2D. For joint training on 2D and 3D datasets, we alternate sampling 2D and 3D batches with batch sizes of 3 and 8 per GPU, respectively. We adopt Mask2Former's strategy, using Hungarian matching for matching queries to ground truth instances and supervision losses (Binary Cross-Entropy and DICE loss for mask prediction, Cross-Entropy loss for classification). Note that our model is only trained for instance segmentation, however it can perform semantic segmentation for free at test time. We refer to Mask2Former \cite{m2f} for more details.

% \todo{add important training details}

% We load all pre-trained weights from checkpoints of Mask2Former \cite{m2f} trained on COCO \cite{coco}, and train all parameters of our model including the pre-trained as well as the new parameters from cross-view layers. When training in 3D scenes, we feed a sequence of $N$ consecutive frames to our model where $N$ is typically 25 frames. At test time, we feed all images in the scene to our model (there are 90 images on average per scene in scannet). We use open vocabulary mask decoding when training jointly on 2D and 3D datasets, and vanilla closed-vocabulary decoding otherwise. We train until convergence on 2 40 GB A100s/ 48GB A6000s with an effective batch size of 6 in 3D and 16 in 2D. When training jointly on 2D and 3D datasets, we interleave sampling 2D and 3D batches with their batch sizes being 3 and 8 per GPU respectively. We follow Mask2Former's strategy of Hungarian matching the queries to ground truth instances and supervision losses (Binary cross-entropy and DICE loss for mask prediction, cross entropy loss for classification). Note that our model is only trained for instance segmentation, however it can perform semantic segmentation for free at test time. We refer to Mask2Former \cite{m2f} for more details.


%Our model predicts a mask segment and a class distribution for each query. We follow previous work on object detection and segmentation \cite{detr,m2f} to find the optimal matching of predicted and ground-truth instances using the Hungarian algorithm. Specifically, given $N$ queries (thus $N$ predict instances) and $M$ ground-truth instances (typically $N>>M$), the algorithm matches $1-1$ $M$ out of $N$ predicted instances to ground-truth instances, while the rest $N-M$ predictions are left unmatched. The matching algorithm takes into consideration both how similar the masks look as well as how well the class distributions match. For the $M$ matched predictions we supervise the predicted mask using a combination of L2 and DICE loss \cite{m2f}, and supervise the class using a softmax loss against the target class of the matched ground-truth. For the $N-M$ unmatched predictions, we supervise the predicted class distribution using a softmax loss against a ``no object" class.
%Note that our model is only trained for instance segmentation, however it can perform semantic segmentation for free at test time. We refer to Mask2Former \cite{m2f} for more details.


%For predicting the instance class, Mask2Former employs an MLP over the queries to map it to the dimension of the number of classes which is supervised by a softmax loss. However, this limits the model to a fixed set of vocabulary and hence makes it difficult to train jointly on datasets with different category labels. Hence, to make our model capable of training on multiple datasets, we follow the model design of BUTD-DETR \cite{butd}, GLIP \cite{glip} and X-Decoder \cite{}. In addition to visual input, we supply our model with a \textit{detection prompt} which is simply the object categories chained together in a sentence (For eg. Chair. Table. Sofa.). We encode this sentence with RoBERTA \cite{}. In the transformer decoder, the object queries attend to the encoded language tokens, then to the visual tokens, and finally self-attend to each other. Finally, to predict the object class, these queries do a dot-product with the language tokens to predict one logit per sentence token. We then mean the logits of all the sentence tokens belonging to a particular object class token to obtain a per-class logits which can be supervised by the vanilla cross-entropy loss.

%Popular 3D benchmarks \cite{} provide a pointcloud and labels sitting on them and evaluate for the segmentation output on the given pointcloud. As explained in the related work section, these datasets are typically created by collecting RGB and depth information through camera sensors, estimating poses through bundle reconstruction and then reconstructing a mesh for the scene. After some further post-processing and cleaning steps, humans label the obtained mesh. Then, pointclouds and labels are sampled from these meshes which are used in the benchmark. Since our model operates on RGB-D input, instead of a pointcloud, we unproject the features to 3D using the sensor data, transfer features to the mesh sampled pointcloud and train and evaluate on the mesh sampled pointcloud. 

% \todo{Also mention that we can do instance and semantic segmentation jointly same as m2f}

% \subsection{Background}
% Discuss Mask2Former and Mask3D (which is simply Mask2Former but 3D conv instead of resnet; 3D positional embeddings in transformer instead of 2D)

% \subsection{Our Model}
% Model closely follows Mask2Former, following are the changes:
% \subsubsection{Point Attention Network}

% Quite similar as Point transformer and Point Transformer v2, but we implement it by using vanilla multihead attention instead of fancier stuff proposed previously. And this attention can be shared between both 2D and 3D with the only difference in how you get the K neighbours and the positional embeddings. Also, mention that positional embeddings are relative to KNN center

% We have these panet layers between resnet layers and during upsampling. 

% \subsection{Positional Embedding}
% 3D learnable positional embedding when we have depth; 2D fourier embeddings when only 2D

% \subsection{Interpolation / Voxelization}
% can skip, but bilinear interpolation and trilinear interpolation in 3D was a very very important change quantitatively. This change happened at upsampling layers as well as "masked cross attention" in decoder head. Voxelization was an important change too to make things efficient and independent of view density.

% \subsection{Open Vocabulary}
% - form detection prompts and do dot-product 



==> oldintro.tex <==
\section{Introduction}

\topic{the paradox of 2d pretraining not helping and the sota being small within domain pointcloud models}

There has been a lot of recent excitement and research interest in porting 2D foundational image features for 3D scene understanding \cite{}, with models that either directly lift  pre-trained 2D image features \icte{} using sensed depth into 3D feature clouds \cite{} or voxelised 3D feature maps \cite{}, or fir per scene 3D differentiable models, such as Nerfs, to render 2D foundational image feature maps \cite{}, distilling 2D feature backbones to the per scene 3D model.  

%It's a paradix, that such 

Recent advances in single 2D image understanding have little  benefited  understanding of 3D scenes so far.   
(Pre-)training 2D image feature backbones to caption \cite{CLIP,captiongenerator} or generate  images \cite{dalle,MAE} large scale  has been instrumental for state of the art 2D image segmentation and labelling, while the state-of-the-art in parsing 3D scene pointclouds in established benchmarks of ScanNet and are in-domain trained point cloud models that operate directly on RGB-D point cloud data and do not use any image feature pre-training, such as Mask3D \cite{}. %Foundational CLIP models have been used for zero-shot 3D scene labelling by lifting and aggregating CLIP features across views with sensed depth, yet, they quite under perform in-domain small scale  3d point cloud models. %Nerfing 2d foundational features is time 
Methods that assign 2d foundational features to 3D points either by direct lifting using densed depth or by  distilling 2D foundational image features to per scene fitted NerF models quite under perform in-domain small scale  3d point cloud models. Moreover, they only address 3D point semantic labelling since 3d object detection requires more nuanced information fusion across multiple image views. %The later \cite{} are also very expensive to fit per scene and require multiple views available. %are time consumeing to fit oper scene, need all views available and under use pretrained foundational 2D models and distill them in multi-view input through training a parametric 3d model per scene to render 2d pretrain features, is fitted per scene and take multiple minutes to fit,and requires dense image coverage, resulting in much sub par zero shot performance.

%Why this paradoxical behaviour?



\topic{the claimed differences between 3d and 2d and its consequences in 3d perception}
%It has been argued that 2D and 3D perception are indeed quite different, and
It has been argued that  building foundational models of 3d perception  would   require a very large 3D (complete multiview data) annotated data, currently unavailable \cite{}.
%Indeed, 3D perception research has evolved often independently from 2d image one, proposing architectures that consume 3D point cloud data, such as PointNet, Minkowsi convolutions, Swin 3d or 3d point transformers that are types of graph neural networks on 3D point graphs. 
Indeed, it is unimaginable that a model can be shared across both 2d and 3d visual understanding, given that images and point clouds are very different in nature, and models have been developed to consume one or the other type of input. This perceived difference has as a consequence 3d point cloud architectures though  capable in parsing objects with distinctive shapes, they cannot reason about surface patterns, such as wall paintings, screen  or 2D photo content, parsimonious in today's environments, while 2D models cannot exploit the presence of depth. %Furthermore, there is a discontinuity between single image perception models and full complete 3d point clouds used for training and evaluation in established benchmarks \cite{}: what happens when few views are available?



%In this paper we ask the question
%This is quite paradoxical that large scale image recognition pre-training cannot assist 3d scene perception, or, when it does, it much underperforms in-domain small scale trained models. How can 2D image models 

%that in the era of foundational models, where large-scale pre-trained models can be finetuned or prompted in so many tasks, such zero shot models for 3D perception that use pre-trained CLIP features lifted to 3D using sensed depth are quite below the performamce of in-domain trained 3d point cloud models (\todo{how much?}

%Why this paradoxical behaviour arises

%captioning models, detectiors or segmentor neural models  trained on large and diverse datasets with varying amount of supervision

%from weak captions to object segments and labels, 

%Currently, 3D perception has not benefited from the advances in single image perception.


%So far, research progress on understanding images and understanding 3D scenes, have 

%so: 3d mesh is used as a representation of the scene.

%problem recognizing patterns without a distinctive shape, e.g., these methods wouldnt be able to recognize anything on wall paiting or pictures or computer screen, it is just flat.

%paradox: despite 2d pretraining, they do not achieve SOTA, why?

Currently, 3D perception has not benefited from the advances in single image perception. The state of the art in object detection and seg  
%from multiple calibrated image views 
in established 3D datasets Scannet dataset  does not use any feature pretraining, rather, trains in domain from scratch from an RGB-D 3d pointcloud  processed from sensed  RGB-D images. The methods that use pretrained foundational 2D models and distill them in multi-view input through training a parametric 3d model per scene to render 2d pretrain features, is fitted per scene and take multiple minutes to fit,and requires dense image coverage, resulting in much sub par zero shot performance. It has been argued that a foundational model for 3D perception would simply require a very large 3D (complete multiview data) to work, currently unavailable.  

%Is it that the foundational model principle breaks for 3d perception? 






%Architecture of 3d perception 
%Points:
%2d perception and 3d perception are disjoint:

%1. 3D models run on different input 3D meshes, and do not exploit 2d pretraining-> mask3d SOTA
%2. 2d featurization that run on different views of a multiview scenes, and a cross view late feature pooling -> open scenes very late fusion of information across views
%3. open scene 3D distill 2D features to a 3D RGB-D pointcloud input model. only miou
%Basically: all models that featurize are much below mask3d
%So: this is against foudnational principle: mask3d trains from scratch and gets sota performance.

In this paper, we ask the question: Is 2D and 3D perception indeed that different? After all, a 3D scene pointcloud is simply an accumulation of depth-augmented images from multiple viewpoints, and it is not god-given or benchmark-provided as it appears in today's 3d perception benchmarks. We propose \model{}, a relative position transformer model that can consume both 2D RGB images and a variable number of posed RGB-D images with the sole difference being the positional encoding: in 2D images, the feature positional encoding reflects $(x,y)$ pixel coordinates while in 3D pointclouds the positional encoding reflects $(X,Y,Z)$ 3D scene coordinates. We use relative position attention operations in both 2D and 3D to gain translation invariance, and use K-nn neighborhoods in 3D attention to handle the quadratic explosion. Our 2D feature backbone is large scale pre-trained and then lifted for the 3D cross view transformer. 


We test \model{} in various 3D benchmarks. Our experiments make several key revelations: 
1) The performance of 3D poincloud models, such as Mask3D, varies a lot depnding on whether they are trained and tested on the 3D mesh provided by the benchmark, the 3D point cloud assembled from rendered 3D deth maps, or the pointcloud assembled from sensed RGB-D images, with a continuous degradation in performance. Our model is close to mask3d in given mesh and much outperforms it in the rendered and sensed depth case across datasets.
2) In simulation environments, where depth does not suffer from noise, our model outperforms 3D point cloud models across the board, suggesting that slight misalignments between 3d mesh and sensed RGB-D views may be to blame for performance. We set a new state of the art in \cite{} simply by replacing the per view detector and tracker of the leading method with our 3d perception system
3) Our 3d performance improved when the model is cotrained with 2D data, showing a synergy not only through pretrained features but also through data concatenation
4) Our model improves with higher capacity of the 2D pretrained backbone.


%When mask3d is trained and tested not in the dataset provided mesh 
%First, we show that our model is close to SOTA mask3d 

%We argue what differs between 2d and 3d data is the  additional depth channel that can be , essentially changing the 


%But we argue that 3d and 2d are close. 3d meshes came from images, they are not god given. So, we seek a modle that can consume a variable number of input views and their depth prediction.  how can 2d feature pertaining  

%segmentation as a unified task between 2D and 3D instead of bounding boxes


%In recent years, significant advancements in the field of computer vision have been driven by the scaling up of models and the utilization of vast amounts of data. However, when it comes to 3D data, the challenges of collection and annotation have hindered the progress of scaling up 3D model learning. Unlike their 2D counterparts, 3D models often struggle to generalize effectively across domains. This limitation raises the question of how we can bring 3D and 2D models closer together to enable the direct sharing of data and parameters, given the abundance of labeled 2D data and the availability of robust architectures.

%One popular perspective within the research community suggests moving away from scaling 3D models and instead exploring the use of 2D foundation models to tackle 3D perception. These models focus on freezing the weights learned from 2D data and subsequently employing them per view, with simple fusion techniques applied. While they show impressive results in zero-shot settings, they significantly underperform compared to domain-specific 3D architectures when tasked with processing 3D information. Consequently, it becomes crucial to investigate how multiview methods can be developed to bridge the performance gap and enable the sharing of 2D-3D data and architectures.

%While previous attempts have been made to employ 2D-based multiview methods on datasets such as ScanNet, their conclusions have shown that these methods are generally inferior to dedicated 3D models. \cite{} showed that when using rendered views, larger camera field of view and active view sampling, the performance of these methods can approach that of domain-specific models. Notably, most of these approaches have focused on semantic segmentation, where the objective is pixel-wise labeling, rather than instance labelling, which requires substantial cross view reasoning to associate same instance of an object across multiple views. In fact, the only RGB-based method available on Instance Segmentation Benchmark of Scannet is MaskRCNN, which was introduced back in 2017. Therefore, in order to develop comprehensive architectures that can effectively share 2D-3D data and architectures, it is essential to study the development of multiview methods capable of achieving comparable performance to 2D models.


%In this work, we aim to take a significant step towards addressing this challenge by proposing a novel multiview RGBD model. Our model achieves close-to-state-of-the-art results on the ScanNet benchmark for both semantic and instance segmentation. Moreover, we demonstrate that our model exhibits better generalization capabilities compared to domain-specific models when dealing with out-of-distribution scenes. Furthermore, our model can be stably trained on both 2D and 3D data, enabling it to process various inputs during testing, including single RGB images, video sequences, and image sequences with depth information. While our approach does not achieve the current state-of-the-art performance, our findings suggest that a multiview RGBD approach holds promise as a viable solution for enhancing 3D perception. Consequently, this approach has the potential to scale 3D perception across diverse classes and facilitate real-world applications.


==> oldintro2.tex <==
\section{Introduction}

\topic{the paradox of 2d pretraining not helping and the sota being small within domain pointcloud models}

There has been a lot of recent excitement and research interest in porting 2D foundational image features to 3D scene understanding \cite{}.
\todo{lets list all different categories of methods that attempt this}
Some methods  lift  pre-trained 2D image features using sensed depth into 3D feature clouds \cite{} or voxelised 3D feature maps \cite{}, and others distil 2D feature backbones to  3D models  such as Nerfs,  fitted per scene to ``render" 2D  image feature maps of pretrained 2D backbones \cite{}.  These efforts are supported by the continual improvement of pre-trained 2D image features through large-scale weakly supervised image captioning  \cite{CLIP,captiongenerator} or  image generation \cite{dalle,MAE}. Empirical evidence shows they are instrumental for state-of-the-art performance in downstream tasks of 2D image segmentation and labelling \cite{}. Paradoxically, and in stark contrast to the 2D domain,  
%Despite these efforts and the , 
the state-of-the-art in 3D instance segmentation and labelling %object detection and pixel labelling 
in established 3D perception benchmarks such as ScanNet, ScanNet200 and Matterport are  models that operate directly on the dataset-provided 3D point clouds and trained in-domain  without using any image featurization and related pre-training \cite{mask3d}. %\todo{do we want to give an example of performamce between lets say openfusion and } %For instance, zero-shot 2D foundational model for 3D only address 3D semnaitc  labelling and obtain such and such score, while an in-domain train Mask3d model attains . 
There are several benefits in foregoing dataset-provided 3D meshes and instead operate directly from the posed RGB-D images. First, %3D mesh 
%that geenrated them:  instead. preprocessing:  processing steps arequite involving and 
in several real-world applications we need agents to function directly from incomplete posed RGB-D input, bypassing involving and time consuming post-processing. Second, it would let us use large pre-trained (foundational) 2D  image backbones for 3D perception. Third, it would bring the research communities of 2D and 3D perception  closer, allowing models to transfer across the two. Yet, getting good results  from raw posed RGB-D data hasn't worked well in these benchmarks  due to misalignments and noise between camera poses and the labelled 3D meshes. %  thus undermining this direction, and  % together by using RGBD and thus could pursue a single architecture. 
This performance gap has nourished the idea that 2D and 3D perception are  very different in nature, and should be addressed with distinct neural models, justified by the fact that images and 3D point clouds are very different in nature.   
%It has been argued that  building foundational models of 3d perception  would   require a very large 3D (complete multiview data) annotated data, currently unavailable \cite{}.
%Indeed, 3D perception research has evolved often independently from 2d image one, proposing architectures that consume 3D point cloud data, such as PointNet, Minkowsi convolutions, Swin 3d or 3d point transformers that are types of graph neural networks on 3D point graphs. 
Indeed, it is unimaginable that a model can be shared across both 2D and 3D visual understanding.
%given that images and 3D point clouds are very different in nature, and so far models have been developed to consume one or the other type of input. 
\todo{Notable exception is omnivore \cite{} but it only addresses the image labelling task, not instance  segmentation and labelling. +++} 


\todo{\model{} can also stand for Omni Dimensional Instance Segmentation if we want to use it}

In this paper, we challenge this view and propose \model{}, a model for 2D and 3D object detection and labelling that can consume both 2D single images and multiview posed RGB-D ones, with SOTA or close to SOTA performance across both 2D and 3D parsing in multiple benchmarks.   
%ask the question: Is 2D and 3D perception indeed that different? After all, a 3D scene pointcloud is simply an accumulation of depth-augmented images from multiple viewpoints, and it is not god-given or benchmark-provided as it appears in today's 3d perception benchmarks. 
 \model{} is a relative position transformer 
 that alternates between 2D within image fusion and 3D cross-image fusion.
 The main difference between 2D and 3D operations is the 
 %can consume both 2D RGB images and a variable number of posed RGB-D images with the sole difference being
 the positional encoding: in 2D images, the feature positional encoding reflects $(x,y)$ pixel coordinates of the 2D token while in multiview RGB-D images the positional encoding reflects $(X,Y,Z)$ 3D scene coordinates of the 3D tokens. We use relative position attention operations in  3D to gain translation invariance to the center of the coordinate system. Our 2D feature backbone is pre-trained in a weakly-supervised fashion. We use $K$-NN neighborhoods in 3D attentions to avoid the quadratic cost of all-to-all attention in 3D. %Our 2D feature backbone is a large  pre-trained and then lifted for the 3D cross view transformer. 


We test \model{} in the COCO 2D object detection benchmark and in the 3D benchmarks of Scannet \cite{}, Scannet200 \cite{}, Matterport \cite{} and S3did \cite{} where it achieves SOTA performance in .... and close to SOTA in ..., while maintaining SOTA 2D COCO meanAP. Our ablations show that cotraining across both 2D and 3D examples helps boost 3D performance, and the model improves with the capacity of the pre-trained backbone. Our model outperforms more naive ways of 2D and 3D feature fusion, without alteration between the two. 
Our comparisons and ablations against 3D point cloud methods \cite{} suggest that their performance varies sugnificantly with the quality of the 3D input point cloud, with \model{} greatly outperforming them when all models use the point cloud assembled from posed RGB-D images directly, in place of the dataset provided 3D mesh.  In the simulation benchmark of ALFRED that does not suffer from misalignments between estimated poses and 3D mesh, our model outperforms 3D point cloud methods and sets a new state-of-the-art in the TEACH instruction following benchmark when used as the 3D detector of a SOTA embodied agent model \cite{}.  
Our comparisons and ablations against methods that lift and average 2D foundational features across views show that though this suffices for 3D point labelling, cross view fusion is essential for 3D object detection, where our model shines over all alternatives. We will make our models and code publicly available upon publication. 

